On Efficient Range-Summability of Ideally IID Random Variables in Two or Higher Dimensions

$d$-dimensional (for $d>1$) efficient range-summability ($d$D-ERS) of random variables (RVs) is a fundamental algorithmic problem that has applications to two important families of database problems, namely, fast approximate wavelet tracking (FAWT) on data streams and approximately answering range-sum queries over a data cube. Whether there are efficient solutions to the $d$D-ERS problem, or to the latter database problem, have been two long-standing open problems. Both are solved in this work. Specifically, we propose a novel solution framework to $d$D-ERS on RVs that have Gaussian or Poisson distribution. Our $d$D-ERS solutions are the first ones that have polylogarithmic time complexities. Furthermore, we develop a novel $k$-wise independence theory that allows our $d$D-ERS solutions to have both high computational efficiencies and strong provable independence guarantees. Finally, we show that under a sufficient and likely necessary condition, certain existing solutions for 1D-ERS can be generalized to higher dimensions.

==> sections/application_________.tex <==

\section{Applications of $\bf{d}$D Gaussian-ERS}\label{sec:introapplication}

In this section, we introduce two important applications of our $d$D Gaussian-ERS solution. 

\subsection{Fast Approximate Wavelet Tracking}\label{sec:FAWT}

The first application is to the problem of fast approximate wavelet tracking (FAWT) on data streams~\cite{onepasswavelet, cormodewavelettracking}. 
Our $d$D Gaussian-ERS solution can be applied in the same way to another provably equivalent problem called space-efficient histogram maintenance (SEHM) on data streams~\cite{dyahist, muthukrishnanhistogram}.
%Since, on data streams, the FAWT problem is provably equivalent to the  problem, here we focus only on how our solution is applied to FAWT with the understanding that it can be applied to SEHM in the same way.HWT-based 

We first introduce the FAWT problem in 1D~\cite{onepasswavelet}, or 1D-FAWT for short.  
In this problem, the precise system state is comprised of a $\Delta$-dimensional vector $\vec{\mathbf{s}}$, each scalar of which is a counter.  
The precise system state at any moment of time is determined by a data stream, in which each data item is an update to 
one such counter (called a {\it point update}) or all counters in a 1D range (called a {\it range update}).  In 1D-FAWT, $\vec{\mathbf{s}}$ is considered
a $\Delta$-dimensional signal vector that is constantly ``on the move'' caused by the updates in the data stream.  
Let $\vec{\mathbf{r}}$ be the ($\Delta$-dimensional) vector of HWT coefficients of $\vec{\mathbf{s}}$. 
Clearly, $\vec{\mathbf{r}}$ is also a ``moving target''.  We denote as $\vec{\mathbf{r}}_t$ the snapshot of $\vec{\mathbf{r}}$ at a time $t$.
In 1D-FAWT, the goal is to closely track (the precise value of) $\vec{\mathbf{r}}$ over time using a {\it sketch}, in the sense that at moment $t$, 
%\textbf{denoting the snapshot of $\vec{\mathbf{r}}$ at this moment as $\vec{\mathbf{r}}_t$}, 
we can recover from the sketch
an estimate $\vec{\mathbf{r}}'_t$ of $\vec{\mathbf{r}}_t$, such that $\|\vec{\mathbf{r}}_t - \vec{\mathbf{r}}'_t\|_2$ is small.   An acceptable solution should use a sketch whose size (space complexity)  is
only $O(\mathrm{polylog}(\Delta))$, and be able to maintain the sketch with a computation time cost of $O(\mathrm{polylog}(\Delta))$ per point or range update.  

The first solution to 1D-FAWT was proposed in~\cite{onepasswavelet}.  It requires the efficient computation of an arbitrary scalar in $H \vec{\mathbf{x}}$, where $H$ is the $\Delta\times\Delta$ Haar matrix (to be defined in~\autoref{sec:1dmath}) and 
$\vec{\mathbf{x}}$ is a $\Delta$-dimensional vector of 4-wise independent Rademacher RVs.
% due to the fact that its tracking (the leading HWT coefficients) operation  that each has the Rademacher distribution
%is performed in the wavelet domain while its sketching operation is implicitly in the time domain.
A key step of this computation is 
to compute a range-sum of 4-wise independent Rademacher RVs (in $1$D), that is used therein as a Tug-of-War (ToW) sketch~\cite{ams} for ``sketching'' the $L_2$ difference (approximation error) between 
the signal vector and its FAWT approximation.
%which was tackled in~\cite{onepasswavelet} using 
An aforementioned ECC-based ERS solution is used therein to tackle this Rademacher-ERS problem. 
%We note this range sum is used in this 1D-FAWT  solution also known as a Tug-of-War (ToW) sketch~\cite{tug-of-war-paper} for estimating the $L_2$ norm of a data stream.
Authors of~\cite{muthukrishnanhistogram} stated that if they could find a solution to this Rademacher-ERS problem in $d$D, then the 1D-FAWT solution in~\cite{onepasswavelet} would become a
$d$D-FAWT solution.  
%However, as mentioned earlier, no multi-dimensional ERS solution has been found until this paper.
The first solution to $d$D-FAWT, proposed in~\cite{cormodewavelettracking}, explicitly bypassed this ERS problem.

We note that the 1D-FAWT solution above continues to work, and its time and space complexities remain the same, 
if we replace the $\vec{\mathbf{x}}$ with a $\Delta$-dimensional vector of 
4-wise independent standard Gaussian RVs.  This is because, with this replacement, the aforementioned ToW sketch becomes a Gaussian Tug-of-War (GToW) sketch (which maps a data item to a 
Gaussian RV instead of a Rademacher RV)~\cite{stabledist},
and ToW and GToW are known to have the same $(\epsilon, \delta)$ accuracy bound~\cite{ams, stabledist} for sketching the $L_2$ norm of a data stream (used here for sketching the 
aforementioned $L_2$ difference). 
Based on this insight, our $d$D Gaussian-ERS solution can be used to construct a $d$D-FAWT solution as follows.  
We simply change, in the {\it contingent} $d$D-FAWT solution proposed in~\cite{onepasswavelet}, the distribution of all $\Delta^d$ underlying 4-wise independent RVs 
from Rademacher to Gaussian.  
With this replacement, this {\it contingent} solution will finally work, {\it provided} we can solve the resulting $d$D ERS-Gaussian problem.
% (with underlying Gaussian 
%RVs being 4-wise independent). 
The latter problem is solved by our $k$-wise (with $k=4$ here) independence scheme, to be described in~\autoref{sec:kwise}.  
The resulting $d$D-FAWT solution has the same time and space complexity of $O(\log^d\Delta)$ (ignoring $\epsilon$ and $\delta$ terms)
as that proposed in~\cite{cormodewavelettracking} for achieving the same $(\epsilon, \delta)$ accuracy guarantee.   

%, which  can be solved using  for $d$D Gaussian-ERS.



% This replacement of target distribution works, since any range-sum would have similar distributions before and after.
%\textbf{ [This is on accuracy, not directly on complexity] since any range-sum would have similar distributions (\textbf{random walk vs. Gaussian random walk}) before and after this replacement.}
%With this replacement, the resulting $d$D Gaussian-ERS problem on $4$-wise independent underlying RVs can be solved using our $k$-wise ($k=4$) independence scheme proposed in~\autoref{sec:kwise}.\textbf{seeds of $k$-wise independent hash functions (each of which is very short in practice)}
	
%	using our Gaussian-ERS solution combined with the  (with $k = 4$for this application)  theory }

\subsection{Range-Sum Queries over Data Cube}\label{sec:datacube}
Our second application is to the problem of approximately answering range-sum queries over a data cube~\cite{datacube} that is similarly ``on the move'' propelled by the (point or range) updates that arrive in a stream. 
This problem can be formulated as follows.  The precise system state is comprised of $\Delta^d$ counters, namely $\sigma_{\vec{\mathbf{i}}}$ for $\mathbf{i}\in [0, \Delta)^d$, that are ``on the move''.   
Given a range $[\vec{\mathbf{l}},\vec{\mathbf{u}})$ at moment $t$, the goal is to approximately compute the sum of counter values in this range $C[\vec{\mathbf{l}},\vec{\mathbf{u}})\triangleq \sum_{\vec{\mathbf{i}}\in[\vec{\mathbf{l}},\vec{\mathbf{u}})} \sigma_{\vec{\mathbf{i}}}(t)$, where $\sigma_{\vec{\mathbf{i}}}(t)$ is the value of the counter $\sigma_{\vec{\mathbf{i}}}$ at moment $t$.   %This problem in 1D can be generalized to that in $d$D in the same way as the ERS problem.Until this paper, no solution that satisfies has been found for this problem
A desirable solution to this problem in $d$D should satisfy three requirements (in which multiplicative terms related to the desired $(\epsilon, \delta)$ accuracy bound are ignored).
First, any range-sum query is answered in $O(\mathrm{polylog}(\Delta))$ time. 
Second, its space complexity is $O(\mathrm{polylog}(\Delta))$. 
Third, every point or range update to the system state is processed in $O(\mathrm{polylog}(\Delta))$ time. 
It has been a long-standing open question whether there is a solution to this problem that satisfies 
all three requirements when $d>1$.
For example, solutions producing exact answers (to the range queries)~\cite{ibtehazmdsegmenttree, propolyne, shiftsplit} all require $O(\Delta^d \log\Delta)$ space and hence do not satisfy the second requirement;
and Haar+ tree~\cite{haarplustree} works only on static data, and hence does not satisfy the third requirement.
%Indeed, whether such a desirable solution exists has been a long-standing open problem.


In 1D, a solution that satisfies all three requirements (with $d=1$) was proposed in~\cite{onepasswavelet, dyahist}.
It involves 
1D-ERS computations on $4$-wise independent underlying RVs where the target distribution is either Gaussian or Rademacher, which are tackled using 
a DST-based~\cite{dyahist} or a ECC-based~\cite{onepasswavelet} 1D-ERS solution, respectively.  As shown in~\cite{onepasswavelet, dyahist}, this range-sum query solution can be readily generalized to $d$D if the ERS computations above can be performed in $d$D. 
This gap is again filled by our $k$-wise ($k=4$) independence scheme for $d$D Gaussian-ERS, 
resulting in the first $d$D solution that satisfies all three requirements, all with $O(\log^d\Delta)$ (time or space) complexity (ignoring $\epsilon$ and $\delta$ terms).

In the resulting $d$D solution, we maintain $O(\log (1/\delta)/\epsilon^2)$ (independent instances of) sketches that each ``sketches" the content (counter values) of the data cube.
Here we describe only one such sketch, which we denote as $A$, since these sketches are statistically and functionally identical.  
At any time $t$, $A(t)$ should track the current system state, namely ($\sigma_{\vec{\mathbf{i}}}(t)$)'s, as follows:  $A(t) \triangleq \sum_{\vec{\mathbf{i}}\in[0, \Delta)^d}\sigma_{\vec{\mathbf{i}}}(t) X_{\vec{\mathbf{i}}}$.
Here $X_{\vec{\mathbf{i}}}$ for $\mathbf{i}\in [0, \Delta)^d$ are (realizations of) a set of $\Delta^d$ $4$-wise independent standard Gaussian underlying RVs that have
one-to-one correspondences with the set of $\Delta^d$ counters as follows:  Each $X_{\vec{\mathbf{i}}}$ is associated with a counter $\sigma_{\vec{\mathbf{i}}}$.  
If we implement these $\Delta^d$ RVs using (an instance of) our $d$D Gaussian-ERS solution, then we can keep the value of $A(t)$ up-to-date, with a time complexity of $O(\log^d\Delta)$
per point or range update (to the system state).  
%, we need to first fix $\Delta^d$ $4$-wise independent standard Gaussian underlying RVs, each of which say $X_{\vec{\mathbf{i}}}$
%is associated with a counter say $\sigma_{\vec{\mathbf{i}}}$.  Then, for each point or range update to the system state (the values of these counters), we 
%adjust the sketch value accordingly so that it is always equal to $A \triangleq \sum_{\vec{\mathbf{i}}\in[0, \Delta)^d}\sigma_{\vec{\mathbf{i}}}(t) X_{\vec{\mathbf{i}}}$ at any time $t$.  
Then, given a query range $[\vec{\mathbf{l}},\vec{\mathbf{u}})$ at time $t$, we estimate the range-sum of counters 
$C[\vec{\mathbf{l}},\vec{\mathbf{u}})$ from the sketch $A(t)$ using $A(t)\cdot S[\vec{\mathbf{l}},\vec{\mathbf{u}})$ as the estimator.
These $O(\log (1/\delta)/\epsilon^2)$ estimators, one obtained from each sketch, are then combined to produce a final estimation that has the following accuracy guarantee (that is the 
same as in the 1D case).
%By the guarantees in~\cite{onepasswavelet}, with $O(\log (1/\delta)/\epsilon^2)$ space complexity and the same amount of time complexity per point or range update, the range-sum  $C[\vec{\mathbf{l}},\vec{\mathbf{u}})$ can be estimated 
With probability at least $1-\delta$, the final estimation deviates from the actual value of $C[\vec{\mathbf{l}},\vec{\mathbf{u}})$ by at most $\epsilon \sqrt{V[\vec{\mathbf{l}},\vec{\mathbf{u}})}\|\bm{\sigma}\|_2$, where $V[\vec{\mathbf{l}},\vec{\mathbf{u}}) \triangleq \prod_{j=1}^{d}(u_j - l_j)$ is the number of counters in the query range, and $ \|\bm{\sigma}(t)\|_2 \triangleq \left(\sum_{\vec{\mathbf{i}}\in[0, \Delta)^d} \sigma^2_{\vec{\mathbf{i}}}(t)\right)^{1/2}$ is the $L_2$ norm of the system state. 
Since each sketch uses an independent $d$ Gaussian-ERS scheme instance, our $d$D solution satisfies all three aforementioned requirements all with $O(\log^d\Delta \log (1/\delta)/\epsilon^2)$ time and space complexity.

\begin{comment}
As what will be an important observation throughout this paper, the range-sum  $C[l, u) = \langle\bm{\sigma}, \mathbbm{1}_{[l, u)}\rangle$, the inner product between the system state and a $\Delta$-dimensional indicator vector $\mathbbm{1}_{[l, u)}$ whose $i^{th}$ element is $1$ if $l\leq i\leq u$ and is $0$ otherwise. If we think of $\mathbbm{1}_{[l, u)}$ as the system state after a range update $([l, u), 1)$, then the corresponding accumulator is $S[l, u)$ and can be efficiently computed with ERS solutions. By~\cite{alonjoinsize}, the product $A\cdot S[l, u)$ estimates $C[l, u)$ with the following guarantees.
%\textcolor{red}{this lemma is copied from and needs re-phrasing}


\begin{lemma}[]
	Let $\hat{C}[l,u)$ be the median of $O(\log(1/\delta))$ means, each averaging over $O(1/\epsilon^2)$ independent copies of  
	%[orginal]	Let $\hat{C}[l, u]$ be the $O(\log (1/\delta))$-wise median of $O(1/\epsilon^2)$-wise mean of independent copies of
	$A\cdot S[l, u) = \left(\sum_{i=0}^{\Delta-1}\sigma_i X_i\right)\cdot \left(\sum_{i=l}^{u}X_i\right)$, then $|\hat{C}[l, u) - C[l, u)| \leq \epsilon \sqrt{u-l+1} \|\bm{\sigma}\|_2$ with probability $1-\delta$.
\end{lemma}
Moreover, the range-sum queries on $d$-dimensional universes, in which the goal is to estimate $C[\mathbf{l}, \mathbf{u}) = \sum_{ \mathbf{i}\in[\mathbf{l}, \mathbf{u})}\sigma_{\mathbf{i}}$, can be similarly answered assuming the underlying RVs of the GToW sketch is generated by our $d$D-ERS solution. 
}
\end{comment}
% \textbf{In our solution, the three $O(\mathrm{polylog}(\Delta))$ terms in the three requirements are all $O(\log^d\Delta)$}.

%, , and requires only $4$-wise independence among the underlying RVs.  a $d$D Gaussian- or Rademacher-ERS solution is available.  Our $d$D Gaussian-ERS solution   fills this gap and results .  
%, and a typical query is to estimate a certain function of the current counter values. This general problem and has been extensively studied recently~\cite{laumdrangequery, agarwalrangesearching}, usually with an additional assumption that the nonzero counters  $\sigma_{\mathbf{i}}$ are  very sparse. %$\bm{\sigma}_{\mathbf{i}}=0$ for all but a few disjoint counters.combined with the $4$-wise independence theory
%In the sequel, we focus on solutions for the ``data cube'', in which  nonzero counters $\sigma_{\vec{\mathbf{i}}}$ are generally dense.
%(old) In the sequel, we adopt the opposite ``data cube'' assumption that nonzero counters $\sigma_{\mathbf{i}}$ are generally dense. We consider only  of additive updates and range-sum queries on data cubes 

\begin{comment}

 ==========
 [old ToW - GToW]
 
For the ease of presentation, we assume the system state is static (without updates) for now. 
%This range-sum query problem is reduced to ERS as stated in~\cite{onepasswavelet}. 
The solution employs a sketch comprised of multiple independent accumulators. The sketch may take one of the two variants: tug-of-war (ToW)~\cite{ams} where the underlying RVs are Bernoulli RVs defined above and Gaussian tug-of-war (GToW) where the underlying RVs are standard Gaussian RVs. 
For each accumulator, we fix $\Delta^d$ 4-wise independent standard Gaussian RVs $X(\mathbf{i})$ for $\mathbf{i}\in[0, \Delta)^d$, and maintain the value $A\triangleq \sum_{i\in[0,\Delta)^d} X_{\mathbf{i}}\sigma_{\mathbf{i}}$. To answer a range-sum query on $[\mathbf{l}, \mathbf{u})$, we multiply each accumulate with a corresponding range-sum of underlying RVs $S[\mathbf{l}, \mathbf{u}) \triangleq \left(\sum_{\mathbf{i}\in[\mathbf{l}, \mathbf{u})}X_\mathbf{i}\right)$. For this purpose, a $d$D-ERS solution  is necessary to quickly generate $S[\mathbf{l}, \mathbf{u})$ in order to meet requirement (i) above. The following lemma show the accuracy guarantees of the sketch-based scheme.

\begin{lemma}[\cite{onepasswavelet}]
	Let $\hat{C}[\mathbf{l}, \mathbf{u}) $ be the median of $O(\log(1/\delta))$ means, each averaging over $O(1/\epsilon^2)$ independent copies of  
	$A\cdot S[\mathbf{l}, \mathbf{u}) $, then $|\hat{C}[\mathbf{l}, \mathbf{u}) - C[\mathbf{l}, \mathbf{u})| \leq \epsilon \|\mathbbm{1}_{[\mathbf{l}, \mathbf{u})}\|_2 \|\bm{\sigma}\|_2$ with probability $1-\delta$, where $\|\bm{\sigma}\|_2 = (\sum_{\mathbf{i}\in[0,\Delta)^d}\sigma_{\mathbf{i}}^2)^{1/2}$ is the $L_2$ norm of the system state.
\end{lemma}

With our $d$D-ERS solution, the  accumulator $A$ can be efficiently updated for both point and range updates. 
%Since these accumulators are independent and functionally equivalent, it suffices to describe the update procedure for one such accumulator $A$, which is initialized to $0$ at the beginning.  (say, a point update without loss of generality)
Given a point update $(\mathbf{i}_t, \delta_t)$, we only need to generate $X_{\mathbf{i}_t}$ and increment $A$ by $\delta_t  X_{\mathbf{i}_t}$. Given a range update $([\mathbf{l}_t, \mathbf{u}_t), \delta_t)$, we need to generate the range-sum $S[\mathbf{l}_t, \mathbf{u}_t)$ using our ERS solution and increment $A$ by $\delta_t S[\mathbf{l}_t, \mathbf{u}_t)$.
\end{comment}


%, where $X_{i_t}$ is one of the underlying RVs that is fixed after being generated on-demand
%for the first time and is associated with the counter $\sigma_{i_t}$. 
%The sketch may take one of the following two flavors depending on the distribution of the underlying RVs. When they are single-step random walks, this sketch is called tug-of-war (ToW)~\cite{ams}; when they are standard Gaussian RVs, it is called Gaussian tug-of-war (GToW). 
%The two variants are statistically close in the following sense: After the entire data stream has passed, $A = \sum_{i=0}^{U-1}\sigma_i X_i$ is (at least approximately) distributed as a Gaussian RV $\mathcal{N}(0, \|\bm{\sigma}\|_2^2)$ by the central limit theorem, where $\|\bm{\sigma}\|_2$ is the $L_2$ norm of the system states. Note that when the underlying RVs are generated by ERS solutions, this sketch naturally supports range-updates. 
%As what will be an important observation throughout this paper, the range-sum  $C[l, u) = \langle\bm{\sigma}, \mathbbm{1}_{[l, u)}\rangle$, the inner product between the system state and a $\Delta$-dimensional indicator vector $\mathbbm{1}_{[l, u)}$ whose $i^{th}$ element is $1$ if $l\leq i\leq u$ and is $0$ otherwise. If we think of $\mathbbm{1}_{[l, u)}$ as the system state after a range update $([l, u), 1)$, then the corresponding accumulator is $S[l, u)$ and can be efficiently computed with ERS solutions. By~\cite{alonjoinsize}, the product $A\cdot S[l, u)$ estimates $C[l, u)$ with the following guarantees.
%\textcolor{red}{this lemma is copied from and needs re-phrasing}


\begin{comment}
[\textbf{Merge with '' no solution satisfies three requirements''}] Finally, we note that various versions of this problem in $d$D have many applications in online analytical processing (OLAP) systems~\cite{datacube} and have been extensively studied in the literature. 
None of these solutions satisfy all three requirements.  
For example, solutions producing exact answers (to the range queries)~\cite{ibtehazmdsegmenttree, propolyne, shiftsplit} all require $O(\Delta^d \log\Delta)$ space and hence do not satisfy the second requirement;
and Haar+ tree~\cite{haarplustree} works only on static data, and hence does not satisfy the third requirement.
\end{comment}
%Note that the reason that these wavelet-based schemes like~\cite{propolyne} satisfy (i) (efficient range-sum query) is similar to the reason that our wavelet-based ERS solution efficiently generates range-sums. However, these works lack an important ``simulation part'' that is to generate wavelet coefficients $\langle \psi, X\rangle$  for different wavelet functions $\psi$, as we have already mentioned in the first application. Since they do not provide any new views on that simulation problem over the aforementioned wavelet tracking papers~\cite{dyahist, muthukrishnanhistogram, cormodewavelettracking}, we still  consider our wavelet-based ERS solution a nontrivial contribution.  %covered all wavelet-related views , yet they did not publish the same idea as how we generate $\langle \psi, X\rangle$. Therefore, we 


 %(old) Before describing the sketch-based scheme, we have to clarify that it is not our contribution but is from~\cite{onepasswavelet}  and the idea is originally from~\cite{ams}. Also, it is more natural to use this original domain sketch and our $d$D-ERS solution than our ``nearest neighbor''~\cite{cormodewavelettracking}, which is completely in the wavelet domain.\textbf{Mention original versions use Rademacher RVs, but we do not know how to generate $4$-wise independent Rademacher range-sums on high dimensions???}

% For simplicity, we describe this problem in one dimension; our description is readily generalizable to multiple dimensions. Given a range-sum query on $[l, u)$, the goal is to estimate $C[l, u)\triangleq \sum_{i=l}^{u-1} \sigma_i$, the sum of counter values whose indices fall in this range. We have to clarify here the range-sum is taken on the counters instead of RVs as in the definition of ERS.




%Moreover, the range-sum queries on $d$-dimensional universes, in which the goal is to estimate $C[\mathbf{l}, \mathbf{u}) = \sum_{ \mathbf{i}\in[\mathbf{l}, \mathbf{u})}\sigma_{\mathbf{i}}$, can be similarly answered assuming the underlying RVs of the GToW sketch is generated by our $d$D-ERS solution. 


%Besides ToW and GToW, another type of sketch called count-min can also answer range-sum queries on either one dimension~\cite{countmin} or multiple dimensions~\cite{friedmanboxquery}. This solution uses $O(\log^d\Delta\log (1/\delta)/\epsilon)$ space and $O(\log^d\Delta\log (1/\delta))$ time per update, and estimates $|\hat{C}[l, u] - C[l, u]| \leq 2\epsilon \log_2\Delta \|\bm{\sigma}\|_1$ with probability $1-\delta$. Under a mildly strong assumption that $\|\bm{\sigma}\|_1$ is on the same order as $\sqrt{\Delta} \|\bm{\sigma}\|_2$, which holds if $O(\Delta)$ counters $\sigma_i$ have values that are nonzero and much less than $\Delta$, the count-min sketch achieves a shorter update time by a factor of $O(\epsilon^2)$ at the cost of using more space by a factor of $O(\epsilon\log^d\Delta)$. However, this solution does not support range-update of the system state.



%the Haar wavelet and the Gaussian-DST. In the above relationship, the Haar wavelet transform was applied to the underlying RVs. The paper that first proposed the Gaussian-DST also mentioned the Haar wavelet, but it focused on transforming an input signal by the Haar wavelet, and the Gaussian-DST is the  of a data streaming algorithm that supports this transformation. In this paper, we will elaborate on SEHM, which naturally generalizes to multidimensional settings~\cite{muthukrishnanhistogram}. In SEHM, ERS solutions are used to answer range-sum queries, ERS solutions are used in theA typical data streaming query is to estimate a certain function of the counter values after the updates caused by all the data items in the data stream are committed to the system state.  , with the underlying RVs distributed in the stable family, generalizes the classic $L_p$-norm estimation algorithm in~\cite{stabledist} to handle range-updates~\cite{1ddyadic}, $d$D-ERS generalizes it to handle range-updates in multidimensional universes.This generalization could potentially lead to many exciting applications. For example, 


%In this work, we make three major contributions.  First, we propose a novel dyadic simulation framework and develop three novel ERS solutions, namely Gaussian-DST, Cauchy-DST and RW-DST, using it.  
%Our solutions are better than all existing ones in that the underlying RVs thus generated are mutually independent empirically and can be made provably so at a small
%cost.Second, we develop a novel $k$-wise independent theory that allows our ERS solutions to have both high computational efficiencies and strong provableindependence guarantees.Third, we propose two nontrivial applications of our ERS solutions, in the areas of data streaming and ANNS, respectively.

\begin{comment}
as novel applications of our ERS solutions, we propose two range-efficient data streaming algorithms for processing streams with arbitrary range-updates.  
Fourth, as a novel application of our ERS solution for Gaussian to ANNS-$L_1$, 
we explain why in RW-LSH we cannot compute random walks using EH3, and propose GRW-LSH as its replacement that has nearly the same efficacy, 
requires virtually zero storage, and is usually more efficient computationally. 

{\color{red} [old] In this work, we make three major contributions.  First, we propose a novel dyadic simulation framework and develop three novel ERS solutions using it.  
Our solutions are better than all existing ones in that the underlying RVs thus generated are mutually independent empirically and can be made provably so at a small
cost.
Second, as novel applications of our ERS solutions, we propose two range-efficient data streaming algorithms for processing streams with arbitrary range-updates.  
Third, as a novel application of our ERS solution for Gaussian to ANNS-$L_1$, 
we explain why in RW-LSH we cannot compute random walks using EH3, and propose GRW-LSH as its replacement that has nearly the same efficacy, 
requires virtually zero storage, and is usually more efficient computationally. }
\end{comment}



==> sections/application_copy.tex <==

\section{Applications of $\bf{d}$D Gaussian-ERS}\label{sec:introapplication}

In this section, we introduce two important applications of our $d$D Gaussian-ERS solution. 

\subsection{Fast Approximate Wavelet Tracking}\label{sec:FAWT}

The first application is to the problem of fast approximate wavelet tracking (FAWT) on data streams~\cite{onepasswavelet, cormodewavelettracking}. 
%Our $d$D Gaussian-ERS solution can be applied in the same way to another problem called space-efficient approximate histogram maintenance (SEAHM) on data streams~\cite{dyahist, muthukrishnanhistogram} that is equivalent to FAWT on 1D, but harder on $d$D.
%Since, on data streams, the FAWT problem is provably equivalent to the  problem, here we focus only on how our solution is applied to FAWT with the understanding that it can be applied to SEHM in the same way.HWT-based 
We first introduce the FAWT problem in 1D~\cite{onepasswavelet}, or 1D-FAWT for short.  
In this problem, the precise system state is comprised of a $\Delta$-dimensional vector $\vec{\mathbf{s}}$, each scalar of which is a counter.  
The precise system state at any moment of time is determined by a data stream, in which each data item is an update to 
one such counter (called a {\it point update}) or all counters in a 1D range (called a {\it range update}).  In 1D-FAWT, $\vec{\mathbf{s}}$ is considered
a $\Delta$-dimensional signal vector that is constantly ``on the move'' caused by the updates in the data stream.  
Let $\vec{\mathbf{r}}$ be the ($\Delta$-dimensional) vector of HWT coefficients of $\vec{\mathbf{s}}$. 
Clearly, $\vec{\mathbf{r}}$ is also a ``moving target''.  We denote as $\vec{\mathbf{r}}_t$ the snapshot of $\vec{\mathbf{r}}$ at a time $t$.
In 1D-FAWT, the goal is to closely track (the precise value of) $\vec{\mathbf{r}}$ over time using a {\it sketch}, in the sense that at moment $t$, 
%\textbf{denoting the snapshot of $\vec{\mathbf{r}}$ at this moment as $\vec{\mathbf{r}}_t$}, 
we can recover from the sketch
an estimate $\vec{\mathbf{r}}'_t$ of $\vec{\mathbf{r}}_t$, such that $\|\vec{\mathbf{r}}_t - \vec{\mathbf{r}}'_t\|_2$ is small.   An acceptable solution should use a sketch whose size (space complexity)  is
only $O(\mathrm{polylog}(\Delta))$, and be able to maintain the sketch with a computation time cost of $O(\mathrm{polylog}(\Delta))$ per point or range update.  

The first solution to 1D-FAWT was proposed in~\cite{onepasswavelet}.  It requires the efficient computation of an arbitrary scalar in $H \vec{\mathbf{x}}$, where $H$ is the $\Delta\times\Delta$ Haar matrix (to be defined in~\autoref{sec:1dmath}) and 
$\vec{\mathbf{x}}$ is a $\Delta$-dimensional vector of 4-wise independent Rademacher RVs.
% due to the fact that its tracking (the leading HWT coefficients) operation  that each has the Rademacher distribution
%is performed in the wavelet domain while its sketching operation is implicitly in the time domain.
A key step of this computation is 
to compute a range-sum of 4-wise independent Rademacher RVs (in $1$D), that is used therein as a Tug-of-War (ToW) sketch~\cite{ams} for ``sketching'' the $L_2$ difference (approximation error) between 
the signal vector and its FAWT approximation.
%which was tackled in~\cite{onepasswavelet} using 
An aforementioned ECC-based ERS solution is used therein to tackle this Rademacher-ERS problem. 
%We note this range sum is used in this 1D-FAWT  solution also known as a Tug-of-War (ToW) sketch~\cite{tug-of-war-paper} for estimating the $L_2$ norm of a data stream.
Authors of~\cite{muthukrishnanhistogram} stated that if they could find a solution to this Rademacher-ERS problem in $d$D, then the 1D-FAWT solution in~\cite{onepasswavelet} would become a
$d$D-FAWT solution.  
%However, as mentioned earlier, no multi-dimensional ERS solution has been found until this paper.
The first solution to $d$D-FAWT, proposed in~\cite{cormodewavelettracking}, explicitly bypassed this ERS problem.

We note that the 1D-FAWT solution above continues to work, and its time and space complexities remain the same, 
if we replace the $\vec{\mathbf{x}}$ with a $\Delta$-dimensional vector of 
4-wise independent standard Gaussian RVs.  This is because, with this replacement, the aforementioned ToW sketch becomes a Gaussian Tug-of-War (GToW) sketch (which maps a data item to a 
Gaussian RV instead of a Rademacher RV)~\cite{stabledist},
and ToW and GToW are known to have the same $(\epsilon, \delta)$ accuracy bound~\cite{ams, stabledist} for sketching the $L_2$ norm of a data stream (used here for sketching the 
aforementioned $L_2$ difference). 
Based on this insight, our $d$D Gaussian-ERS solution can be used to construct a $d$D-FAWT solution as follows.  
We simply change, in the {\it contingent} $d$D-FAWT solution proposed in~\cite{onepasswavelet}, the distribution of all $\Delta^d$ underlying 4-wise independent RVs 
from Rademacher to Gaussian.  
With this replacement, this {\it contingent} solution will finally work, {\it provided} we can solve the resulting $d$D Gaussian-ERS problem.
% (with underlying Gaussian 
%RVs being 4-wise independent). 
The latter problem is solved by our $k$-wise (with $k=4$ here) independence scheme, to be described in~\autoref{sec:kwise}.  
The resulting $d$D-FAWT solution has the same time and space complexity of $O(\log^d\Delta)$
as that proposed in~\cite{cormodewavelettracking} for achieving the same accuracy guarantee.   

%, which  can be solved using  for $d$D Gaussian-ERS.



% This replacement of target distribution works, since any range-sum would have similar distributions before and after.
%\textbf{ [This is on accuracy, not directly on complexity] since any range-sum would have similar distributions (\textbf{random walk vs. Gaussian random walk}) before and after this replacement.}
%With this replacement, the resulting $d$D Gaussian-ERS problem on $4$-wise independent underlying RVs can be solved using our $k$-wise ($k=4$) independence scheme proposed in~\autoref{sec:kwise}.\textbf{seeds of $k$-wise independent hash functions (each of which is very short in practice)}
	
%	using our Gaussian-ERS solution combined with the  (with $k = 4$for this application)  theory }

\subsection{Range-Sum Queries over Data Cube}\label{sec:datacube}
Our second application is to the problem of approximately answering range-sum queries over a data cube~\cite{datacube} that is similarly ``on the move'' propelled by the (point or range) updates that arrive in a stream. 
This problem can be formulated as follows.  The precise system state is comprised of $\Delta^d$ counters, namely $\sigma_{\vec{\mathbf{i}}}$ for $\mathbf{i}\in [0, \Delta)^d$, that are ``on the move''.   
Given a range $[\vec{\mathbf{l}},\vec{\mathbf{u}})$ at moment $t$, the goal is to approximately compute the sum of counter values in this range $C[\vec{\mathbf{l}},\vec{\mathbf{u}})\triangleq \sum_{\vec{\mathbf{i}}\in[\vec{\mathbf{l}},\vec{\mathbf{u}})} \sigma_{\vec{\mathbf{i}}}(t)$, where $\sigma_{\vec{\mathbf{i}}}(t)$ is the value of the counter $\sigma_{\vec{\mathbf{i}}}$ at moment $t$.   %This problem in 1D can be generalized to that in $d$D in the same way as the ERS problem.Until this paper, no solution that satisfies has been found for this problem
A desirable solution to this problem in $d$D should satisfy three requirements (in which multiplicative terms related to the desired $(\epsilon, \delta)$ accuracy bound are ignored).
First, any range-sum query is answered in $O(\mathrm{polylog}(\Delta))$ time. 
Second, its space complexity is $O(\mathrm{polylog}(\Delta))$. 
Third, every point or range update to the system state is processed in $O(\mathrm{polylog}(\Delta))$ time. 
It has been a long-standing open question whether there is a solution to this problem that satisfies 
all three requirements when $d>1$.
For example, solutions producing exact answers (to the range queries)~\cite{ibtehazmdsegmenttree, propolyne, shiftsplit} all require $O(\Delta^d \log\Delta)$ space and hence do not satisfy the second requirement;
and Haar+ tree~\cite{haarplustree} works only on static data, and hence does not satisfy the third requirement.
%Indeed, whether such a desirable solution exists has been a long-standing open problem.


In 1D, a solution that satisfies all three requirements (with $d=1$) was proposed in~\cite{onepasswavelet, dyahist}.
It involves 
1D-ERS computations on $4$-wise independent underlying RVs where the target distribution is either Gaussian or Rademacher, which are tackled using 
a DST-based (in~\cite{dyahist}) or a ECC-based (in~\cite{onepasswavelet}) 1D-ERS solution, respectively.  
As shown in~\cite{onepasswavelet, dyahist}, this range-sum query solution can be readily generalized to $d$D if the ERS computations above can be performed in $d$D. 
This gap is again filled by our $k$-wise ($k=4$) independence scheme for $d$D Gaussian-ERS, 
resulting in the first $d$D solution that satisfies all three requirements, all with $O(\log^d\Delta)$ (time or space) complexity (ignoring $\epsilon$ and $\delta$ terms).

In the resulting $d$D solution, we maintain $O(\log (1/\delta)/\epsilon^2)$ (independent instances of) sketches that each ``sketches'' the content (counter values) of the data cube.
Here we describe only one such sketch, which we denote as $A$, since these sketches are statistically and functionally identical.  
At any time $t$, $A(t)$ should track the current system state, namely ($\sigma_{\vec{\mathbf{i}}}(t)$)'s, as follows:  $A(t) \triangleq \sum_{\vec{\mathbf{i}}\in[0, \Delta)^d}\sigma_{\vec{\mathbf{i}}}(t) X_{\vec{\mathbf{i}}}$.
Here $X_{\vec{\mathbf{i}}}$ for $\mathbf{i}\in [0, \Delta)^d$ are (realizations of) a set of $\Delta^d$ $4$-wise independent standard Gaussian underlying RVs that have
one-to-one correspondences with the set of $\Delta^d$ counters as follows:  Each $X_{\vec{\mathbf{i}}}$ is associated with a counter $\sigma_{\vec{\mathbf{i}}}$.  
If we implement these $\Delta^d$ RVs using (an instance of) our $d$D Gaussian-ERS solution, then we can keep the value of $A(t)$ up-to-date, with a time complexity of $O(\log^d\Delta)$
per point or range update (to the system state).  
%, we need to first fix $\Delta^d$ $4$-wise independent standard Gaussian underlying RVs, each of which say $X_{\vec{\mathbf{i}}}$
%is associated with a counter say $\sigma_{\vec{\mathbf{i}}}$.  Then, for each point or range update to the system state (the values of these counters), we 
%adjust the sketch value accordingly so that it is always equal to $A \triangleq \sum_{\vec{\mathbf{i}}\in[0, \Delta)^d}\sigma_{\vec{\mathbf{i}}}(t) X_{\vec{\mathbf{i}}}$ at any time $t$.  
Then, given a query range $[\vec{\mathbf{l}},\vec{\mathbf{u}})$ at time $t$, we estimate the range-sum of counters 
$C[\vec{\mathbf{l}},\vec{\mathbf{u}})$ from the sketch $A(t)$ using $A(t)\cdot S[\vec{\mathbf{l}},\vec{\mathbf{u}})$ as the estimator.
These $O(\log (1/\delta)/\epsilon^2)$ estimators, one obtained from each sketch, are then combined to produce a final estimation that has the following accuracy guarantee (that is the 
same as in the 1D case).
%By the guarantees in~\cite{onepasswavelet}, with $O(\log (1/\delta)/\epsilon^2)$ space complexity and the same amount of time complexity per point or range update, the range-sum  $C[\vec{\mathbf{l}},\vec{\mathbf{u}})$ can be estimated 
With probability at least $1-\delta$, the final estimation deviates from the actual value of $C[\vec{\mathbf{l}},\vec{\mathbf{u}})$ by at most $\epsilon \sqrt{V[\vec{\mathbf{l}},\vec{\mathbf{u}})}\|\bm{\sigma}\|_2$, where $V[\vec{\mathbf{l}},\vec{\mathbf{u}}) \triangleq \prod_{j=1}^{d}(u_j - l_j)$ is the number of counters in the query range, and $ \|\bm{\sigma}(t)\|_2 \triangleq \left(\sum_{\vec{\mathbf{i}}\in[0, \Delta)^d} \sigma^2_{\vec{\mathbf{i}}}(t)\right)^{1/2}$ is the $L_2$ norm of the system state. 
Since each sketch uses an independent $d$D Gaussian-ERS scheme instance, our $d$D solution satisfies all three aforementioned requirements, all with $O(\log^d\Delta \log (1/\delta)/\epsilon^2)$ time and space complexity.

\subsection{A Closer Comparison with Related Work}

In this section, per referees' requests, we provide an in-depth comparison of this work with prior works on 1D-FAWT~\cite{onepasswavelet, dyahist}, 
on $d$D-FAWT~\cite{cormodewavelettracking}, and on 1D data 
cube~\cite{dyahist}.  
%Its purpose is to assess how far each prior work had come towards formulating and solving this $d$D range summability problem to and explain why in some cases.
%We first provide a short story here.  
%This explanation highlights the unique contributions of this work in terms of four detachments.

We start with explaining how the $d$D-FAWT solution proposed in~\cite{cormodewavelettracking} manages to avoid confronting the $d$D-ERS problem.  
The $d$D-FAWT solution~\cite{cormodewavelettracking} maintains ToW sketches for groups of wavelet coefficients in the wavelet domain.  
As explained earlier, each ToW sketch ``measures'' the $L_2$ norm (and hence the total energy by squaring) of such a group.     
By the property of HWT, each point or range update to the system state in the time domain translates into $O(\log^d \Delta)$ updates to the sketches the wavelet domain;
we also use this property in our solution to keep its time complexity below $O(\log^d \Delta)$ as shown in~\autoref{sec:waveletdd}.  
To solve the $d$D-FAWT using these sketches in the wavelet domain, we need only to identify the groups that are (hierarchical) ``$L_2$ heavy hitters''~\cite{cormodewavelettracking}.   
In~\cite{cormodewavelettracking}, a binary search tree built on these sketches is used to search for such ``$L_2$ heavy hitters'' in $O(\log \Delta\cdot \log\log \Delta???)$ time.  
Since this $d$D-FAWT solution~\cite{cormodewavelettracking} does not involve computing the range sums of the Rademacher RVs underlying the ToW sketches, 
it does not need to formulate or solve any ERS problem.
%these RVs only need to be 4-wise independent as required by ToW.  

In comparison, should we try to extend the 1D-FAWT solution proposed in~\cite{onepasswavelet}, which maintains the ToW sketches
in the time domain, to $d$D without the aforementioned Rademacher-by-Gaussian replacement, 
%we would be faced with a $d$D Rademacher-ERS problem.  
the underlying Rademacher RVs would have to be efficiently range-summable to keep the time complexity of each point or range update to the sketches low.   
However, this appears to be a tall order for now:  For $d>1$, no ECC-based Rademacher-ERS solution has ever been found as explained earlier, and a DST-based 
Rademacher-ERS solution is unlikely to exist, as we will show in \autoref{sec:infeasibility} and \autoref{sec:casenegative}.

{\bf JFM: I think you can "avoid" ERS by moving everything, including the input streams and the query ranges into the wavelet domain. That is exactly what our algorithm is doing. Cormode used 4-wise independent ToW sketches. If they had proposed i.i.d. Gaussian sketches, then their solution would be identical to ours. We want to stress that although this idea might sound obvious, nobody has ever realized that this wavelet-based solution is also an ERS solution.}
A referee asked whether the 1D data cube solution proposed in~\cite{onepasswavelet, dyahist} can be extended to $d$D using the same ERS avoidance strategy of 
maintaining the sketches in the wavelet domain as used in~\cite{cormodewavelettracking}.  The answer to this question is negative for the following reason.  
The ToW or GToW sketches are used in all three FAWT and data cube solutions~\cite{onepasswavelet, dyahist, cormodewavelettracking}, whether the sketches are maintained 
in the time domain or in the wavelet domain.  
As explained in \autoref{sec:datacube}, to use such a sketch $A(t)$ for answering a data cube query, we have to compute 
$A(t)\cdot S[\vec{\mathbf{l}},\vec{\mathbf{u}})$, which involves computing the range sum $S[\vec{\mathbf{l}},\vec{\mathbf{u}})$.  

Now we highlight a key difficulty that we believe has prevented authors of~\cite{onepasswavelet, dyahist, muthukrishnanhistogram} from solving the $d$D-ERS problem and 
extending their FAWT and data cube solutions from 1D to $d$D:  The Rademacher or Gaussian RVs underlying the sketches need to be both 4-wise independent
and efficiently range-summable.  Authors of~\cite{onepasswavelet, muthukrishnanhistogram} tried to extend a magic hash function, that induces such Rademacher RVs in 1D, to $d$D.
However, as explained extending it to $d$D, a $d$D Rademacher-ERS solution is unlikely to exist.  Authors of~\cite{dyahist} proposed the 1D-DST that laid the foundation of this work 
and our prior work~\cite{1ddyadic}.  A key innovation of~\cite{dyahist} is that the 1D-ERS is achieved via a 1D-DST instead of a magic hash function.  
However, their DST-based 1D Gaussian-ERS solution still relies on a magic hash function, called Nisan's PRG (Pseudorandom Generator)~\cite{nisan}, to provide 4-wise independence among the underlying Gaussian RVs.
The use of Nisan's PRG~\cite{nisan} however restricts the applicability and the extensibility of the 1D-DST approach, since Nisan's PRG provides independence guarantees only for memory-constrained applications
such as data streaming~\cite{stabledist}.  It is also not clear whether the 1D-DST approach powered by Nisan's PRG can be extended to $d$D.  
In comparison, in this work, the $d$D-DST (that exists for Gaussian and Poisson) data structure is engineered to provide $k$-wise independence among underlying RVs.
Each underlying hash function, one the other hand, only needs to output $k$-wise independent hash values, which as mentioned earlier is easy to achieve.  
Note $k$-wise independence among underlying RVs is fundamentally different and much harder to attain than $k$-wise independence among hash values (produced by a hash function), since 
each underlying RV can be a weighted sum of $O(\log^d \Delta)$ such hash values, as we will elaborate in \autoref{sec:kwise}.  
{\bf JFM: I think the difficulty here is that the underlying RVs need to be range-summable, while the hash values are not.}

Finally, we state a key difference between this work and~\cite{onepasswavelet, dyahist, muthukrishnanhistogram, cormodewavelettracking} with respect to wavelets.  In this work, ERS is the end and wavelets is the means,
whereas in~\cite{onepasswavelet, dyahist, muthukrishnanhistogram} it is the other way around.  In~\cite{cormodewavelettracking}, wavelets is the end, but~\cite{cormodewavelettracking} cleverly avoids using 
ERS as the means as just explained.


\begin{comment}

since in our aforementioned proposed solution to $d$D-FAWT that extends

the (Gaussian) RVs underlying the GToW sketches 
requires


aforementioned extension of 


If we maintain an aforementioned ToW-like sketch for FAWT in the time domain, to accommodate a range-update (... ) we need ERS to bring the complexity within ???.  
In the wavelet domain, a range update causes ??? updates to the sketch of the wavelet coefficienct, so the job becomes 
a (special form) heavy hitter one.  Search for hierractical heavy hitters on this sketch does not involving computing the range sum of sketching RVs.  
The sketch for L2 heavy hitter, still needs 4-wise independent, but not 4-wise plus range summability.
This is a much easier problem than we have to solve.

how the 1D-FAWT solutions~\cite{onepasswavelet,dyahist} 

One key gap is that existing solutions do not separate exact or approximate 4-wise indepence from range summability. 
Third:  detach the hashing mechanism from the solution.  The solution works, with storing the previously generated wavelet coefficients, as long as the sufficient condition is satisfied.  
The k-wise theory is independent of the solution.  When using it to replace the stored coefficients, we can reduce storage.  In comparison, in [7] the hashing solution and the sketch solution
is integrated.  They use 1 and -1 generated from ECCs such as Reed-Muller.  

We show whether ERS summability is possible depends only on the dist of the underlying RV, and orthogonal to how much space we need.  
The latter, if doable due to the dist being nice, depends on the level of independence sought.  When only k-wise independence is needed, 
we can do it using ... k-wise hash functions.  Any k-wise hash functions are ok.  We do not need them to be range-summable.  

In prior work, wavelet is the end goal, and range-summability is the means.  In our scheme, range-summability is the end goal.
It works for wavelet, not working using wavelet.  The means is actually DST, and wavelet is just a special case when the dist is gaussian.
It happens to take the wavelet form when the dist is Gaussian.  The Poisson one has nothing to do with Wavelet.

The dist used is Rademacher for the Tug-of-War thing.  Distance is "two hops":  (1) Rademacher is not doable, (2) 4-wise plus range summability

wavelet is searchable at dD:  whose hierarchical structure allows for binary search, 

[4] cannot be used to solve data cube because [4] avoids the computation of range sum, since it only needs to estimate the L2 norm of a 
dyadic range if it is relatively (to the size of the range) heavy, which does not involve any range sum computaiton .  However, for data cube, we have to multiply a range sum S[a, b) 
to an L2 sketch of the universe.  So we cannot avoid the computation of S[a, b).  

\end{comment}

%general heavy histogram is not searchable at dD:  >1D is NP complete and PTAS exists only for 2D 

%The 1D FAWT paper [7] Gilbert ...  

%First:  detach the ERS oracle from the original problem (or the sketch/application that uses it)     in-house => general purpose.    In the Gilbert paper, the ERS is embedded.  

%Need 4-wise for AMS and ERS for efficient dyadic range query.






\begin{comment}
As what will be an important observation throughout this paper, the range-sum  $C[l, u) = \langle\bm{\sigma}, \mathbbm{1}_{[l, u)}\rangle$, the inner product between the system state and a $\Delta$-dimensional indicator vector $\mathbbm{1}_{[l, u)}$ whose $i^{th}$ element is $1$ if $l\leq i\leq u$ and is $0$ otherwise. If we think of $\mathbbm{1}_{[l, u)}$ as the system state after a range update $([l, u), 1)$, then the corresponding accumulator is $S[l, u)$ and can be efficiently computed with ERS solutions. By~\cite{alonjoinsize}, the product $A\cdot S[l, u)$ estimates $C[l, u)$ with the following guarantees.
%\textcolor{red}{this lemma is copied from and needs re-phrasing}


\begin{lemma}[]
	Let $\hat{C}[l,u)$ be the median of $O(\log(1/\delta))$ means, each averaging over $O(1/\epsilon^2)$ independent copies of  
	%[orginal]	Let $\hat{C}[l, u]$ be the $O(\log (1/\delta))$-wise median of $O(1/\epsilon^2)$-wise mean of independent copies of
	$A\cdot S[l, u) = \left(\sum_{i=0}^{\Delta-1}\sigma_i X_i\right)\cdot \left(\sum_{i=l}^{u}X_i\right)$, then $|\hat{C}[l, u) - C[l, u)| \leq \epsilon \sqrt{u-l+1} \|\bm{\sigma}\|_2$ with probability $1-\delta$.
\end{lemma}
Moreover, the range-sum queries on $d$-dimensional universes, in which the goal is to estimate $C[\mathbf{l}, \mathbf{u}) = \sum_{ \mathbf{i}\in[\mathbf{l}, \mathbf{u})}\sigma_{\mathbf{i}}$, can be similarly answered assuming the underlying RVs of the GToW sketch is generated by our $d$D-ERS solution. 
}
\end{comment}
% \textbf{In our solution, the three $O(\mathrm{polylog}(\Delta))$ terms in the three requirements are all $O(\log^d\Delta)$}.

%, , and requires only $4$-wise independence among the underlying RVs.  a $d$D Gaussian- or Rademacher-ERS solution is available.  Our $d$D Gaussian-ERS solution   fills this gap and results .  
%, and a typical query is to estimate a certain function of the current counter values. This general problem and has been extensively studied recently~\cite{laumdrangequery, agarwalrangesearching}, usually with an additional assumption that the nonzero counters  $\sigma_{\mathbf{i}}$ are  very sparse. %$\bm{\sigma}_{\mathbf{i}}=0$ for all but a few disjoint counters.combined with the $4$-wise independence theory
%In the sequel, we focus on solutions for the ``data cube'', in which  nonzero counters $\sigma_{\vec{\mathbf{i}}}$ are generally dense.
%(old) In the sequel, we adopt the opposite ``data cube'' assumption that nonzero counters $\sigma_{\mathbf{i}}$ are generally dense. We consider only  of additive updates and range-sum queries on data cubes 

\begin{comment}

 ==========
 [old ToW - GToW]
 
For the ease of presentation, we assume the system state is static (without updates) for now. 
%This range-sum query problem is reduced to ERS as stated in~\cite{onepasswavelet}. 
The solution employs a sketch comprised of multiple independent accumulators. The sketch may take one of the two variants: tug-of-war (ToW)~\cite{ams} where the underlying RVs are Bernoulli RVs defined above and Gaussian tug-of-war (GToW) where the underlying RVs are standard Gaussian RVs. 
For each accumulator, we fix $\Delta^d$ 4-wise independent standard Gaussian RVs $X(\mathbf{i})$ for $\mathbf{i}\in[0, \Delta)^d$, and maintain the value $A\triangleq \sum_{i\in[0,\Delta)^d} X_{\mathbf{i}}\sigma_{\mathbf{i}}$. To answer a range-sum query on $[\mathbf{l}, \mathbf{u})$, we multiply each accumulate with a corresponding range-sum of underlying RVs $S[\mathbf{l}, \mathbf{u}) \triangleq \left(\sum_{\mathbf{i}\in[\mathbf{l}, \mathbf{u})}X_\mathbf{i}\right)$. For this purpose, a $d$D-ERS solution  is necessary to quickly generate $S[\mathbf{l}, \mathbf{u})$ in order to meet requirement (i) above. The following lemma show the accuracy guarantees of the sketch-based scheme.

\begin{lemma}[\cite{onepasswavelet}]
	Let $\hat{C}[\mathbf{l}, \mathbf{u}) $ be the median of $O(\log(1/\delta))$ means, each averaging over $O(1/\epsilon^2)$ independent copies of  
	$A\cdot S[\mathbf{l}, \mathbf{u}) $, then $|\hat{C}[\mathbf{l}, \mathbf{u}) - C[\mathbf{l}, \mathbf{u})| \leq \epsilon \|\mathbbm{1}_{[\mathbf{l}, \mathbf{u})}\|_2 \|\bm{\sigma}\|_2$ with probability $1-\delta$, where $\|\bm{\sigma}\|_2 = (\sum_{\mathbf{i}\in[0,\Delta)^d}\sigma_{\mathbf{i}}^2)^{1/2}$ is the $L_2$ norm of the system state.
\end{lemma}

With our $d$D-ERS solution, the  accumulator $A$ can be efficiently updated for both point and range updates. 
%Since these accumulators are independent and functionally equivalent, it suffices to describe the update procedure for one such accumulator $A$, which is initialized to $0$ at the beginning.  (say, a point update without loss of generality)
Given a point update $(\mathbf{i}_t, \delta_t)$, we only need to generate $X_{\mathbf{i}_t}$ and increment $A$ by $\delta_t  X_{\mathbf{i}_t}$. Given a range update $([\mathbf{l}_t, \mathbf{u}_t), \delta_t)$, we need to generate the range-sum $S[\mathbf{l}_t, \mathbf{u}_t)$ using our ERS solution and increment $A$ by $\delta_t S[\mathbf{l}_t, \mathbf{u}_t)$.
\end{comment}


%, where $X_{i_t}$ is one of the underlying RVs that is fixed after being generated on-demand
%for the first time and is associated with the counter $\sigma_{i_t}$. 
%The sketch may take one of the following two flavors depending on the distribution of the underlying RVs. When they are single-step random walks, this sketch is called tug-of-war (ToW)~\cite{ams}; when they are standard Gaussian RVs, it is called Gaussian tug-of-war (GToW). 
%The two variants are statistically close in the following sense: After the entire data stream has passed, $A = \sum_{i=0}^{U-1}\sigma_i X_i$ is (at least approximately) distributed as a Gaussian RV $\mathcal{N}(0, \|\bm{\sigma}\|_2^2)$ by the central limit theorem, where $\|\bm{\sigma}\|_2$ is the $L_2$ norm of the system states. Note that when the underlying RVs are generated by ERS solutions, this sketch naturally supports range-updates. 
%As what will be an important observation throughout this paper, the range-sum  $C[l, u) = \langle\bm{\sigma}, \mathbbm{1}_{[l, u)}\rangle$, the inner product between the system state and a $\Delta$-dimensional indicator vector $\mathbbm{1}_{[l, u)}$ whose $i^{th}$ element is $1$ if $l\leq i\leq u$ and is $0$ otherwise. If we think of $\mathbbm{1}_{[l, u)}$ as the system state after a range update $([l, u), 1)$, then the corresponding accumulator is $S[l, u)$ and can be efficiently computed with ERS solutions. By~\cite{alonjoinsize}, the product $A\cdot S[l, u)$ estimates $C[l, u)$ with the following guarantees.
%\textcolor{red}{this lemma is copied from and needs re-phrasing}


\begin{comment}
[\textbf{Merge with '' no solution satisfies three requirements''}] Finally, we note that various versions of this problem in $d$D have many applications in online analytical processing (OLAP) systems~\cite{datacube} and have been extensively studied in the literature. 
None of these solutions satisfy all three requirements.  
For example, solutions producing exact answers (to the range queries)~\cite{ibtehazmdsegmenttree, propolyne, shiftsplit} all require $O(\Delta^d \log\Delta)$ space and hence do not satisfy the second requirement;
and Haar+ tree~\cite{haarplustree} works only on static data, and hence does not satisfy the third requirement.
\end{comment}
%Note that the reason that these wavelet-based schemes like~\cite{propolyne} satisfy (i) (efficient range-sum query) is similar to the reason that our wavelet-based ERS solution efficiently generates range-sums. However, these works lack an important ``simulation part'' that is to generate wavelet coefficients $\langle \psi, X\rangle$  for different wavelet functions $\psi$, as we have already mentioned in the first application. Since they do not provide any new views on that simulation problem over the aforementioned wavelet tracking papers~\cite{dyahist, muthukrishnanhistogram, cormodewavelettracking}, we still  consider our wavelet-based ERS solution a nontrivial contribution.  %covered all wavelet-related views , yet they did not publish the same idea as how we generate $\langle \psi, X\rangle$. Therefore, we 


 %(old) Before describing the sketch-based scheme, we have to clarify that it is not our contribution but is from~\cite{onepasswavelet}  and the idea is originally from~\cite{ams}. Also, it is more natural to use this original domain sketch and our $d$D-ERS solution than our ``nearest neighbor''~\cite{cormodewavelettracking}, which is completely in the wavelet domain.\textbf{Mention original versions use Rademacher RVs, but we do not know how to generate $4$-wise independent Rademacher range-sums on high dimensions???}

% For simplicity, we describe this problem in one dimension; our description is readily generalizable to multiple dimensions. Given a range-sum query on $[l, u)$, the goal is to estimate $C[l, u)\triangleq \sum_{i=l}^{u-1} \sigma_i$, the sum of counter values whose indices fall in this range. We have to clarify here the range-sum is taken on the counters instead of RVs as in the definition of ERS.




%Moreover, the range-sum queries on $d$-dimensional universes, in which the goal is to estimate $C[\mathbf{l}, \mathbf{u}) = \sum_{ \mathbf{i}\in[\mathbf{l}, \mathbf{u})}\sigma_{\mathbf{i}}$, can be similarly answered assuming the underlying RVs of the GToW sketch is generated by our $d$D-ERS solution. 


%Besides ToW and GToW, another type of sketch called count-min can also answer range-sum queries on either one dimension~\cite{countmin} or multiple dimensions~\cite{friedmanboxquery}. This solution uses $O(\log^d\Delta\log (1/\delta)/\epsilon)$ space and $O(\log^d\Delta\log (1/\delta))$ time per update, and estimates $|\hat{C}[l, u] - C[l, u]| \leq 2\epsilon \log_2\Delta \|\bm{\sigma}\|_1$ with probability $1-\delta$. Under a mildly strong assumption that $\|\bm{\sigma}\|_1$ is on the same order as $\sqrt{\Delta} \|\bm{\sigma}\|_2$, which holds if $O(\Delta)$ counters $\sigma_i$ have values that are nonzero and much less than $\Delta$, the count-min sketch achieves a shorter update time by a factor of $O(\epsilon^2)$ at the cost of using more space by a factor of $O(\epsilon\log^d\Delta)$. However, this solution does not support range-update of the system state.



%the Haar wavelet and the Gaussian-DST. In the above relationship, the Haar wavelet transform was applied to the underlying RVs. The paper that first proposed the Gaussian-DST also mentioned the Haar wavelet, but it focused on transforming an input signal by the Haar wavelet, and the Gaussian-DST is the  of a data streaming algorithm that supports this transformation. In this paper, we will elaborate on SEHM, which naturally generalizes to multidimensional settings~\cite{muthukrishnanhistogram}. In SEHM, ERS solutions are used to answer range-sum queries, ERS solutions are used in theA typical data streaming query is to estimate a certain function of the counter values after the updates caused by all the data items in the data stream are committed to the system state.  , with the underlying RVs distributed in the stable family, generalizes the classic $L_p$-norm estimation algorithm in~\cite{stabledist} to handle range-updates~\cite{1ddyadic}, $d$D-ERS generalizes it to handle range-updates in multidimensional universes.This generalization could potentially lead to many exciting applications. For example, 


%In this work, we make three major contributions.  First, we propose a novel dyadic simulation framework and develop three novel ERS solutions, namely Gaussian-DST, Cauchy-DST and RW-DST, using it.  
%Our solutions are better than all existing ones in that the underlying RVs thus generated are mutually independent empirically and can be made provably so at a small
%cost.Second, we develop a novel $k$-wise independent theory that allows our ERS solutions to have both high computational efficiencies and strong provableindependence guarantees.Third, we propose two nontrivial applications of our ERS solutions, in the areas of data streaming and ANNS, respectively.

\begin{comment}
as novel applications of our ERS solutions, we propose two range-efficient data streaming algorithms for processing streams with arbitrary range-updates.  
Fourth, as a novel application of our ERS solution for Gaussian to ANNS-$L_1$, 
we explain why in RW-LSH we cannot compute random walks using EH3, and propose GRW-LSH as its replacement that has nearly the same efficacy, 
requires virtually zero storage, and is usually more efficient computationally. 

{\color{red} [old] In this work, we make three major contributions.  First, we propose a novel dyadic simulation framework and develop three novel ERS solutions using it.  
Our solutions are better than all existing ones in that the underlying RVs thus generated are mutually independent empirically and can be made provably so at a small
cost.
Second, as novel applications of our ERS solutions, we propose two range-efficient data streaming algorithms for processing streams with arbitrary range-updates.  
Third, as a novel application of our ERS solution for Gaussian to ANNS-$L_1$, 
we explain why in RW-LSH we cannot compute random walks using EH3, and propose GRW-LSH as its replacement that has nearly the same efficacy, 
requires virtually zero storage, and is usually more efficient computationally. }
\end{comment}



==> sections/introduction_jx_________.tex <==
\section{Introduction}\label{sec:intro}

Efficient range-summability (ERS) of ideally i.i.d. random variables (RVs) is a fundamental algorithmic problem that has been studied for nearly two 
decades~\cite{feigenbaum, rusu-jour, dyahist, 1ddyadic}.  This problem has so far been defined only in one dimension (1D) as follows.
Let $X_0, X_1, \cdots, X_{\Delta-1}$ be a list of 
%ideally (mutually) independent
 \emph{underlying RVs} each of which has the same {\it target distribution} $X$.
Here, the (index) universe size $\Delta$ is typically a large number (say $\Delta = 2^{64}$).  
A 1D-ERS problem calls for the following oracle for answering range-sum queries over (realizations of) these underlying RVs.  
At initialization, the oracle chooses a {\it random outcome} $\omega$ from the {\it sample space} $\Omega$, which
{\it mathematically determines} the (values of the) realizations $X_0(\omega), X_1(\omega), \cdots, X_{\Delta-1}(\omega)$;   here the phrase 
“mathematically determines” emphasizes that (an implementation of) the oracle does not actually realize these RVs (and pay the $O(\Delta)$ time cost) at initialization.   
Thereafter, given any query range $[l, u) \triangleq \{l, l+1, \cdots, u-1\}$ that lies in the universe $[0, \Delta)$, the oracle is required to return 
$S[l, u) \triangleq \sum_{i=l}^{u-1}X_i(\omega)$, the sum of the realizations of all underlying RVs in the range.   This requirement is called the \emph{consistency}
requirement, which is one of the two essential requirements for the ERS oracle.   We will show that such an ERS oracle can be efficiently implemented using 
hash functions.  With such an implementation, the outcome $\omega$ corresponds to the seeds of these hash functions. 

%For example, we will describe an oracle based on hash functions. 

The other essential requirement is \emph{correct distribution}, which has two aspects.   
%The consistency requirement is that the returned $S[l, u)$ associated with the outcome $\omega$ (in initialization) must be equal to $\sum_{i=l}^{u-1} X_{i}(\omega)$. 
The first aspect is that the underlying RVs $X_0, X_1, \cdots, X_{\Delta-1}$ each has the same target (marginal) distribution $X$. 
The second aspect is that these RVs should satisfy certain independence guarantees. 
%We will elaborate  later on two kinds of  guarantees: 
As mentioned earlier, ideally these RVs are desired to be all-wise independent, but this comes at a high storage cost as we will elaborate shortly.
In practice, another type of independence guarantee, namely $k$-wise independence (in the sense any subset of $k$ underlying RVs are independent),
%and that induced by Nisan's PRG (pseudorandom generator)~\cite{}, 
is good enough for most applications when $k \ge 4$.   We will show that our solution for ERS in $d>1$ dimensions 
can provide $k$-wise independence guarantee at a small storage cost of $O(\log^d\Delta)$ for an arbitrarily large $k$.  
 
%the first kind is (strict) all-wise independence, and the second kind is $k$-wise independence, which means that any subset of $k$ underlying RVs are independent.

A straightforward but naive way to answer a range-sum query, say on $[l, u)$, is simply to sum up the realization of every underlying RV
$X_l(\omega), X_{l+1}(\omega), \cdots,$ $X_{u-1}(\omega)$ in the query range.
This solution, however, has a time complexity of
$O(\Delta)$ when $u - l$ is $O(\Delta)$.
% which is inefficient computationally when $\Delta$ is large.   
In contrast, an efficient solution should be able to do so with only $O(\mathrm{polylog}(\Delta))$ time complexity.
Indeed, all existing ERS solutions~\cite{calderbank, feigenbaum, rusu-jour, dyahist, 1ddyadic} have $O(\log\Delta)$ time complexity.

\subsection{Related Work on 1D-ERS}\label{sec:1ders}

%The straightforward way of computing range-sums is to generate each of the underlying RVs $X_\mathbf{i}$ in the range individually and then add them up. However, this solution has a time complexity of $O(\Delta^d)$ in the worst case, which is inefficient computationally when $\Delta$ is huge. $\Pr[X = 1] = \Pr[X = -1] = 0.5$,  (\emph{aka}. single-step random walk)



%We first give a brief survey of the related works on the ERS problem in 1D.  

There are in general two families of solutions to the ERS problem in 1D, following two different approaches.  
%All existing solutions have the same asymptotic time complexity of $O(\log \Delta)$.  
The first approach is based on error correction codes (ECC).
Solutions taking this approach include BCH3~\cite{rusu-jour}, EH3~\cite{feigenbaum}, and RM7~\cite{calderbank}. 
This approach has two drawbacks.  First, it works only when the target distribution $X$ is Rademacher.
Second, although it guarantees $3$-wise (in the case of BCH3 and EH3) or $7$-wise (in the case of RM7) independence among the underlying RVs, 
almost all empirical independence beyond that is destroyed. 
In addition, RM7 is very slow in practice~\cite{rusu-jour}.

%, the only existing solution that provides a strict independence guarantee beyond $3$-wise,

The second approach is based on a data structure called dyadic simulation tree (DST), which we will 
describe in~\autoref{sec:dst1D}.  The DST-based approach was first briefly mentioned in~\cite{dyahist} and later fully developed in~\cite{1ddyadic}.  
The DST-based approach is better than the ECC-based approach in two aspects.  First, it
supports a wider range of target distributions including Gaussian, Cauchy, Rademacher~\cite{1ddyadic}, and Poisson (see~\autoref{sec:2ddyasim}). 
Second, it provides stronger independence guarantees at a low computational cost.  
For example, when implemented using the tabulation hashing scheme~\cite{tabulation5wise}, it guarantees $5$-wise independence at a much lower computational
cost than RM7~\cite{1ddyadic}.  We will describe a nontrivial generalization of this result to $2$D in~\autoref{sec:kwise}.



% and this goal has been achieved by~\cite{feigenbaum, rusu-jour, dyahist, 1ddyadic} in 1D.

%[not used] Each such ERS solution generates  a range-sum $S[l, u)$ or an underlying RV $X_{i}$ in a very different way than the naive solution.
%This difference however does not matter since an ERS solution is , given any {\it outcome} $\omega$ in the {\it sample space} $\Omega$ (in probability theory terms),  , where $X_{i}(\omega)$ is the realization of $X_{i}$associated with the same outcome $\omega$.


%For example, our dyadic simulation solution satisfies the first requirement by construction
%and satisfies the second requirement under an idealized assumption (\emph{cf.}~\autoref{lem:correctness}).= (i_1, i_2, \cdots, i_d)^T

\subsection{ERS in Higher Dimensions}

In this work, we formulate the ERS problems in $d>1$ dimensions ($d$D), which we denote as $d$D-ERS, and propose the first-ever solutions to $d$D-ERS.
% for $d>1$.
A $d$D-ERS problem is similarly defined on a $d$-dimensional universe $[0, \Delta)^d$ that contains $\Delta^d$ integral points.  
Each $d$D point $\vec{\mathbf{i}}  \in [0,\Delta)^d$ is associated with
an RV $X_{\vec{\mathbf{i}}}$, and %these $\Delta^d$ underlying RVs are ideally independent and 
every such RV has the same target (marginal) distribution $X$. 
Here, for ease of presentation, we assume $\Delta$ is the same on each dimension and is a power of $2$, but our solutions can work without these two assumptions.
%Given two indices 
Let $\vec{\mathbf{l}}=(l_1, l_2, \cdots, l_d)^T$ and $\vec{\mathbf{u}} = (u_1, u_2, \cdots, u_d)^T$ be two $d$D points in $[0, \Delta)^d$ such that 
$l_j < u_j$ for each dimension $j=1,2,\cdots, d$.  We define $[\vec{\mathbf{l}}, \vec{\mathbf{u}})$ as the $d$D rectangular range ``cornered'' by these two points 
in the sense $[\vec{\mathbf{l}}, \vec{\mathbf{u}}) \triangleq [l_1, u_1)\times [l_2, u_2)\times \cdots\times [l_d, u_d)$, where $\times$ is the Cartesian product. 

A $d$D-ERS problem calls for the following oracle.  At initialization, the oracle chooses an outcome $\omega$ 
that \emph{mathematically determines} the realization $X_{\vec{\mathbf{i}}}(\omega)$ for each $\vec{\mathbf{i}}\in [0, \Delta)^d$. 
Thereafter, given any $d$D range $[\vec{\mathbf{l}}, \vec{\mathbf{u}})$, the oracle returns in $O(\mathrm{polylog}(\Delta))$ time $S[\vec{\mathbf{l}}, \vec{\mathbf{u}}) \triangleq \sum_{\vec{\mathbf{i}}\in [\vec{\mathbf{l}}, \vec{\mathbf{u}})} X_{\vec{\mathbf{i}}}(\omega)$, the sum of the realizations of all underlying RVs in this $d$D range.
%The $d$D-ERS problem is that, given any we need to compute ,
Unless otherwise stated, the vectors that appear in the sequel are assumed to be column vectors. 
We write them in boldface and with a rightward arrow on the top like in ``$\vec{\mathbf{x}}$''.




%Before we describe our $d$D-ERS solutions, we first highlight its importance to database theory.  
Several 1D-ERS solutions have been proposed as an essential building block for efficient solutions to several database problems.  
In two such database problems that we will describe in~\autoref{sec:introapplication}, their 1D solutions, both proposed in~\cite{onepasswavelet}, 
can be readily generalized to $d$D if their underlying 1D-ERS oracles can be generalized to $d$D.  
%\textbf{For example, in one such problem, a $d$D-ERS oracle is needed  so that the algorithm can estimate the range-sum of a data cube from the sketches.}
In fact, in~\cite{muthukrishnanhistogram}, 
authors stated explicitly that the only missing component for their solutions of the 1D database problems to be generalized to 2D was an efficient 
2D-ERS oracle where $X$ is the Rademacher distribution ($\Pr[X = 1] = \Pr[X = 0] = 0.5$, \emph{aka}. single-step random walk).
% but they have never proposed a solution in~\cite{muthukrishnanhistogram} or any of their
%followup works (e.g.,~\cite{muthukrishnan2016}).  In~\cite{cormodewavelettracking}, a different group of researchers solved 
%this database problem in $d$D, by working around this $d$D-ERS problem.  
However, until this paper, \emph{no solution} to any $d$D-ERS problem for $d >1$ 
has been proposed.


%defined as the Cartesian product of $d$ 1D intervals, \ie  $[\mathbf{l}, \mathbf{u}) \triangleq [l_1, u_1)\times [l_2, u_2)\times \cdots\times [l_d, u_d)$, in which each 1D interval $[l, u)$ is the set $\{l, l+1, \cdots, u-1\}$.  
%For example, if $S$ is the range $[\mathbf{l}, \mathbf{u})$, the range-sum $S[\mathbf{l}, \mathbf{u}) = \langle \mathbf{x}, \mathbbm{1}_{[\mathbf{l}, \mathbf{u})} \rangle$.



%efficient range-summability (ERS)=[0, \Delta)^d $$[0, \Delta]\textbf{[from Woodruff] We consider a discrete $d$-dimensional universe$[\Delta]^d = \{0, 1, . . . , \Delta-1\}^d$, where $\Delta$ is the number of discrete coordinates along any dimension,} We consider$d$D-ERS is defined in a $d$-dimensional universe
%In $d$D-ERS, we generate (and fix) $\Delta^d$ (ideally) i.i.d. \emph{underlying RVs} $\{X_{\mathbf{i}}\}$ for each $\mathbf{i} = (i_1, i_2, \cdots, i_d)^T\in [0, \Delta)^d$, each of %which satisfies a given \emph{target distribution} marginally. 




%study a fundamental algorithmic problem that has applications to two important data stream processing and database problems: space-efficient histogram maintenance (SEHM) and range-sum queries on data cubes.
%This algorithmic problem, called $d$-dimensional ($d$D) efficient range-summability (ERS) of random variables (RVs), generalizes 


%the well-established one-dimensional (1D) ERS problem~\cite{feigenbaum, rusu-jour} to higher dimensions, and can be stated as follows.


%lower bounded by $\mathbf{l}$ and upper bounded by $\mathbf{u}$\mathbf{l}\preceq \mathbf{u}$ (which means 

%ERS is a well-established problem on 1D with numerous applications in data streaming such as estimation of $L_1$ difference~\cite{feigenbaum}, estimation of spatial join sizes~\cite{rusu-jour} and space-efficient histogram maintenance (SEHM)~\cite{dyahist}. However, in multidimensional universes, the ERS problem remains unexplored in the literature. 

%$d$D-ERS is an important but challenging problem. The straightforward way of computing range-sums is to generate each of the underlying RVs $X_\mathbf{i}$ in the range individually and then add them up. However, this solution has a time complexity of$O(\Delta^d)$ in the worst case, which is inefficient computationally when either the dimension $d$ or the universe size $\Delta$ is huge. 

%In this work, we propose the first and so far only solution for $d$D-ERS. This solution works only when the underlying RVs have Gaussian or Poisson distribution and runs in $O(\log^d \Delta)$ time. Although the applicable distributions are limited, we believe that our contribution is significant, 
%We consider this a nontrivial contribution even with this restriction, because Gaussian distribution is one of the most widely used distributions for ERS in the literature~\cite{dyahist, 1ddyadic}. We also characterize the condition on the target distribution for dyadic simulation to be feasible for multidimensional ERS. Unfortunately, many common distributions including Cauchy and Bernoulli fail to satisfy the condition, so for them, dyadic simulation in small space is likely to be infeasible. 

%this condition is not satisfied by many common distributions (\eg Cauchy and Bernoulli), on which dyadic simulation is likely to be infeasible in small space.

%so it is likely to be hard to efficiently generate range-sums of empirically independent underlying RVs in small memory space.
%We are also the first to study the infeasibility o f multi-dimensional ERSon general underlying distributions and show that since most common distributions (\eg Cauchy and Bernoulli) lack a ``nice'' independence property, it is likely to be hard to efficiently generate range-sums of empirically independent underlying RVs in small memory space.

%calculate range-sums on an arbitrary dimension independently of other dimensions.
%and because it is a counter-intuitive discovery that its one-dimensional range-sums do not interfere, so the $d$D-ERS problem on it can be algorithmically resolved.
%a range $R(\mathbf{l}, \mathbf{u}) = [l_1, u_1]\times [l_2, u_2] \times \cdots \times [l_d, u_d]$ as the Cartesian product of $d$ discrete intervals (or as $R(\mathbf{l}, \mathbf{u}) =\{\mathbf{i}:l_j \leq i_j \leq u_j, \forall j=1,2, \cdots, d\}$), where  are two indices in $[\Delta]^d$, 


%Let $X_0, X_1, \cdots, X_{U-1}$ be a list of i.i.d. RVs, where the (index) universe size $U$ Given a range $[a, b) \triangleq \{a, a+1, \cdots, b-1\}$ that lies in $[0, U)$, we need ton the one-dimensional case, i
% (per ``requests'' from a database for computing a range-sum 
%application) somehow compute $S[a, b) \triangleq \sum_{i=a}^{b-1}X_i$, the sum of the RVs $X_a, X_{a+1}, \cdots, X_{b-1}$ in the range.. This specific problem has wide applications in ???the dimension the universe sizehave been proposed 

%and provides stronger and more flexible independence guarantees at lower computational costs, as will be elaborated in.

%Ideally, dyadic simulation generates mutually independent i.i.d. RVs, and in practice, it provides three different guarantees on independence that will be specified later. \textbf{which guarantees?}

%\textbf{[need the next sentence?] Also, it is not known in literature whether ECC-based schemes can be generalized to multidimensional ERS.}



%All existing ERS solutions take one of the two approaches.



%Both approaches lead to solutions with time 
%In 1D, ERS is a well-established problem with several existing solutions that significantly reduce the time complexity from $O(\Delta)$ to $O(\log \Delta)$~\cite{feigenbaum, rusu-jour, 1ddyadic}, but on higher dimensions, the ERS problem remains unexplored in the literature. 

%, but neither appears to result in an O(polylog($\Delta$))-time solution for multi-dimensional data.
 
 %none of them has been generalized to O(polylog($\Delta$)) complexity in more than one dimensions.
 
%They all convert
%the focus of these solutions is to sting solutions take two different approaches for this task., such as BCH codes, Hamming codes~\cite{feigenbaum} or Reed-Muller codes~\cite{calderbank}This is a slight abuse of terms, because strictly

%Although not stated in the literature, we have figured out how EH3 can be generalized to solve the ERS problem on multiple dimensions. Since we do not have enough space to make this claim self-contained, we decide to report this result in another following paper.\footnote{ Strictly speaking, ``Bernoulli'' RVs have the distribution $\Pr[X = 1] = \Pr[X = 0] = 0.5$, but here, the ($0$)'s are mapped $(-1)$'s.  Since the mapping will not change the narratives of generating such underlying RVs in the sequel, we slightly abuse the term and also call the mapped distribution ``Bernoulli''.}, which is also known as the ``single-step random walk'' in~\cite{1ddyadic}

%Further, it is not known if these ECC-based schemes can support the ERS problem on more than one dimensions.
%This approach guarantees that the underlying RVs are $k$-wise independent and that the values of the underlying RVs in any dyadic range have a nice pattern such that the range-sum can be efficiently calculated. However, on two dimensions, no such pattern is currently known for the ERS 


%Empirically, the underlying RVs are ``independent enough'' for all practical applications. Theoretically, any range-sum is guaranteed to have the ``correct'' distribution as if it were comprised of mutually independent underlying RVs. 


% in less than a microsecond when is used. In contrast, , takes more than 20 milliseconds to generate a range-sum~\cite{rusu-jour}.



%This reduction is since any non-dyadic range can be split into at most $2\log_2 U$ dyadic ranges. As we will show shortly,  in order to efficiently handle ``strip''-shaped ranges along any dimension, a $d$D-ERS scheme has to somehow assign one-dimensional range-sums on any arbitrary dimension independently of other dimensions. However, this is impossible for general underlying distributions, because the range-sums on different dimensions are almost always interfering with each other.
%This is because are on different dimensions,  us from applying $1$d-ERS on multiple dimensions at the same time.in~\autoref{sec:infeasibility}

%support one-dimensional range-summability simultaneously on all dimensions. 



%For otherexample in which interference of underlying RVs on different dimensions can be  underlying distributions, we have also conducted an ``infeasibility'' study that characterizes why our dyadic simulation solution that works on Gaussian distribution is damaged by the interference from other dimensions.


%We are the first to find out that for Gaussian distribution only, the dyadic simulation solution for $1$D-ERS~\cite{dyahist, 1ddyadic}, called $1$D Gaussian dyadic simulation tree ($1$D Gaussian-DST), has a special equivalent formulation using Haar wavelets, which has been generalized to multiple dimensions in the data streaming literature~\cite{cormodewavelettracking}. We can show that dyadic simulation for Gaussian RVs can also generalized to multiple dimensions using the wavelet formulation.
 %the wavelet formulation generally does not hold. W

%A straightforward but naive solution to this problem, which follows an intuitive ``bottom-up'' %approach, is to generate RVs $X_a, X_{a+1}, \cdots,$ $X_{b-1}$ individually and then add them up.This solution, however, has a time complexity of$O(b - a)$, which is inefficient computationally when the range length $b - a$ is large.   In contrast, an acceptable solution~\cite{feigenbaum, rusu-jour} should be able to do so with only O(polylog($b-a$)) time complexity.  Since  has been  in the data streaming field,  the dyadic simulation solution also .

%This naive solution follows an intuitive ``bottom-up'' approach:  The constituent RVs in the range are individually realized and then added up.solution for $1$D-ERS~\cite{dyahist, 1ddyadic}, called $1$D Gaussian dyadic simulation tree ($1$D Gaussian-DST), $\boldsymbol{d}$ 

\subsection{Our \boldmath{d}D-ERS Solutions}\label{sec:waveletapproach}

In this paper, we propose novel solutions to the two $d$D-ERS problems wherein the target distributions are Gaussian and Poisson respectively. 
We refer to these two problems as $d$D Gaussian-ERS and $d$D Poisson-ERS, respectively. 
Both solutions generalize the corresponding DST-based 1D-ERS solutions to higher dimensions and 
have a low time complexity of $O(\log^d\Delta)$ per range-sum query. 
Our $d$D Gaussian-ERS solution, in particular, is based on the Haar wavelet transform (HWT), since DST is equivalent to HWT when (and only when) the target distribution $X$ is Gaussian,
as will be shown in~\autoref{sec:wavelet1d}. 

Furthermore, we identify a sufficient condition that, if satisfied by the target distribution $X$, 
guarantees that the corresponding DST-based 1D-ERS solution can be generalized to a $d$D-ERS solution.   
We will prove in~\autoref{sec:casepositive} that Gaussian and Poisson are two ``nice'' distributions that satisfy this sufficient condition.
We will also show that, for all such ``nice'' distributions  (including those
we might discover
in the future),
this generalization process (from 1D to $d$D) follows a universal algorithmic framework that can be characterized as the Cartesian product of $d$ DSTs.   
We will also provide
%give evidence that $X$ satisfying this distribution is necessary for this generalization 
strong evidence that $X$ ``being nice'' is likely necessary for this DST generalization (from 1D to $d$D) to be feasible (see~\autoref{sec:infeasibility}).

%-ERS solution with $O(\log^d\Delta)$ time complexity per range-sum query}.

%In this section, we introduce our $d$D-ERS solutions.   Our first solution is for the $d$D-ERS problem where the .  We refer to this problem as .   
%Specifically, we call this problem $d$D Gaussian-ERS when the target distribution is standard Gaussian. A

Unfortunately, so far we have not found any ``nice'' distribution other than Gaussian and Poisson.
%We  strong evidence that being a ``nice'' distribution is likely necessary for the generalization (from 1D to $d$D) to be feasible (see~\autoref{sec:infeasibility}).  
Hence $d$D-ERS for other target distributions remains an open problem, and is likely not solvable by the (generalized) DST approach. 
We emphasize this is not a shortcoming of the DST approach:  That we have obtained computationally efficient solutions in the cases of Gaussian and Poisson 
is nothing short of a miracle, as the $d$D-ERS problem has been open for nearly two decades.    
%In addition, we have strong evidence that none of the ECC-based 1D-ERS solutions can be extended to higher dimensions for providing accurate
%$4$-wise or better independence guarantees.  
Furthermore, 
%since it is well known that a Gaussian range sum can be used wherever a Rademacher range sum is needed (e.g., a Tug-of-War sketch~\cite{} 
%provides the same ``service to upper-layer applications" as a ``Gaussian Tug-of-War sketch"~\cite{}), 
we will show that our $d$D Gaussian-ERS solution leads to computationally efficient solutions to both aforementioned database problems (to be described in Section~\ref{}),
by answering their calls for a $d$D Rademacher-ERS or Gaussian-ERS oracle.  

%answers the ``oracle calls" in both aforementioned
%applications~\cite{} 

%both applications  ``calls for Rademacher $d$D-ERS oracles"  Gaussian distribution and the Rademacher range distrsum in any application, 
%our $d$D Gaussian-ERS solution can serve as the oracle to 

%We believe $d$D-ERS when $X$ is not ``nice" is not solvable by any the aforementioned ECC-based approach 
%suggests that the rigid constraints imposed by the ECC scheme that a would make $d$D-ERS for $d>1$ mathematically impossible.

%Despite this negative result,  our $d$D-ERS solution still has wide applications in data streaming.
%In particular, as we will elaborate in~\autoref{sec:introapplication}, our $d$D Gaussian-ERS oracle solves the following long-standing open problem:
%to approximately answer, in an efficient manner, range-sum queries over a $d$-dimensional dynamic (subject to updates that arrive as a stream) data cube for $d > 1$ [This was in the second %contribution].  
	
%	Given our success in generalizing the DST-based  1D Gaussian-ERS solution to $d$D, we wonder if all DST-based 1D ERS solutions can be generalized to $d$D. 
%As mentioned earlier, in 1D, the DST-based approach that works for multiple target distributions is more general than the HWT-based approach that works only for Gaussian target distribution.(HWT and DST are equivalent here as just explained)
%We wonder whether the more general DST-based approach can be extended to solve the multidimensional ERS problems for target distributions other than Gaussian.}
%	HWT-based approach  that works only for Gaussian target distribution is a special case of the DST-based approach.
%	re are DST-based ERS solutions for target distributions other than Gaussian in 1D, one may naturally wonderwhether there exists a general approach beyond the HWT that can generalize all these solutions to higher dimensions}. %can be generalized to higher dimensions in general.   We find, however, that the answer to this question is likely negative.In particular, we  
%This sufficient condition is so strong that The bad news is that so far we have found only two such ``nice'' distributions, namely Gaussian and Poisson,   and that \textbf{In other words, for distribution other than Gaussian and Poisson, we do not have a $d$D-ERS solution that has $o(\Delta)$ time complexity per range-sum query. }


==================

[old version] In this section, we introduce our $d$D-ERS solutions.  All our solutions generalize the DST-based approach for 1D-ERS and 
have a time complexity of $O(\log^d\Delta)$.   Our first solution is for the $d$D-ERS problem where the target distribution $X$ is standard Gaussian.  
We refer to this problem 
as $d$D Gaussian-ERS.   
%Specifically, we call this problem $d$D Gaussian-ERS when the target distribution is standard Gaussian. 
Our $d$D Gaussian-ERS solution is based on the Haar wavelet transform (HWT), since DST is equivalent to HWT when (and only when) $X$ is Gaussian,
as will be shown in~\autoref{sec:wavelet1d}.


In our solution, to provably guarantee that all the $\Delta^d$ underlying RVs  are independent, in theory we need to make an idealized assumption that we can map
every integer $i\in[0, \Delta^d)$ to a {\it fresh} RV $W_i$ (the $i^{th}$ scalar in the $\Delta^d$-dimensional $\vec{\mathbf{w}}$) independent of other RVs using a truly random hash function~\cite{mitzenmachertrulyrandom}.  
In practice, we can instantiate our solution to 
achieve three different levels of independence guarantees using three different types of more practically implementable hash functions, respectively.   
One such instantiation, called the $k$-wise independence scheme and to be elaborated in~\autoref{sec:kwise}, is another major contribution of this work.  
For any $k > 1$, the 
$k$-wise independence scheme can be configured, by employing $O(\log^{d}\Delta)$ $k$-wise 
independent hash functions to do this mapping (from $i$ to $W_i$), 
to guarantee that the underlying Gaussian RVs are $k$-wise independent.
This scheme makes our Gaussian-ERS solution very practically useful for two reasons. 
First, such a $k$-wise independent hash function in practice requires a very short seed (not longer than a few kilobytes), and each hash operation can be computed in nanoseconds~\cite{univhash, tabulationpower}.
%requires a seed of only $O(\log\Delta)$ bits in length and has only $O(k)$ computational complexity per hashing operation.
%the  (per hashing operation) of  is only  
Second, most applications of ERS only require the underlying RVs to be 4-wise independent~\cite{onepasswavelet, muthukrishnanhistogram}. 
This $k$-wise independence scheme works also for our Poisson-ERS solution (described next).  We however will not explain how it works in this paper, since doing so would involve drilling down to 
the messy and lengthy detail of the Cartesian product of $d>1$ DSTs (since we cannot use the relatively clean and simple $d$D HWT in the Poisson case as just explained).


% although we have yet to find any practical application of the Poisson-ERS problem.

%We will describe two such applications in~\autoref{sec:introapplication}.

%Our Gaussian-ERS solution generalizes the DST-based approach to higher dimensions because, in 1D, a DST is mathematically equivalent to an HWT, as will be shown in~\autoref{sec:dst1D}.
Given our success in generalizing our DST-based (HWT and DST are equivalent here as just explained) 1D Gaussian-ERS solution to $d$D, 
we wonder if all DST-based 1D ERS solutions can be generalized to $d$D.
%As mentioned earlier, in 1D, the DST-based approach that works for multiple target distributions is more general than the HWT-based approach that works only for Gaussian target distribution.
%We wonder whether the more general DST-based approach can be extended to solve the multidimensional ERS problems for target distributions other than Gaussian.}
%	HWT-based approach  that works only for Gaussian target distribution is a special case of the DST-based approach.
%	re are DST-based ERS solutions for target distributions other than Gaussian in 1D, one may naturally wonderwhether there exists a general approach beyond the HWT that can generalize all these solutions to higher dimensions}. %can be generalized to higher dimensions in general.   
We find, however, that the answer to this question is likely negative.
In particular, we have identified a sufficient condition that, if satisfied by the target distribution $X$, 
guarantees that the corresponding DST-based solution for 1D can be generalized to $d$D.
%This sufficient condition is so strong that 
The bad news is that so far 
we have found only two ``nice'' distributions, 
namely Gaussian and Poisson, that satisfy this sufficient condition, and that we have strong evidence that this condition is likely necessary.
Interestingly, for all such ``nice'' distributions (including those
we might discover
in the future),
this generalization process (from 1D to $d$D) follows a universal algorithmic framework.

=================
\begin{comment}
Readers may notice this solution generates (realizes) a range sum $S[\vec{\mathbf{l}}, \vec{\mathbf{u}})$ or an underlying RV $X_{\vec{\mathbf{i}}}$ in a very different way than the naive solution.
This difference however does not matter since an ERS solution is considered correct as long as it satisfies two requirements:  consistency and correct distribution.
The consistency requirement is that, given any outcome $\omega$ in the outcome space $\Omega$, the realization of $S[\vec{\mathbf{l}}, \vec{\mathbf{u}})$ associated with the outcome $\omega$
must be equal to $\sum_{\vec{\mathbf{i}}\in [\vec{\mathbf{l}}, \vec{\mathbf{u}})} X_{\vec{\mathbf{i}}}(\omega)$, where $X_{\vec{\mathbf{i}}}(\omega)$ is the realization of $X_{\vec{\mathbf{i}}}$
associated with the same outcome $\omega$.
The correct distribution requirement is that the underlying RVs thus generated are ideally i.i.d. with distribution $X$.   
Our solution satisfies the consistency requirement by the linearity of HWT, \textbf{as will be shown in~\autoref{sec:1dalgorithm}}, 
and the correct distribution requirement by the first observation above.
Since the first observation is true only when the target distribution is Gaussian,
%For example, our dyadic simulation solution satisfies the first requirement by construction
%and satisfies the second requirement under an idealized assumption (\emph{cf.}~\autoref{lem:correctness}).
this HWT-based solution does not work for any other target distribution. 
\end{comment}


Our $d$D Gaussian-ERS and Poisson-ERS solutions both support two different types of
%satisfies two kinds of 
independence guarantees, at different storage costs.   
The first type is the ideal case in which the $\Delta^d$ underlying RVs are all-wise independent. 
% as will be shown in
As will be shown in~\autoref{sec:dyasim}, we can achieve this ideal case by paying $O(T\log^d \Delta)$ storage cost, where 
$T$ is the total number of range-sum queries to be answered (i.e., $O(\log^d \Delta)$ storage cost per range query). 
%This scheme has the strongest possible guarantee, but may be impractical when the number of range-sum queries is too large.
The second type is also quite strong:  The $\Delta^d$ underlying RVs are $k$-wise independent, where the constant $k$ can be arbitrarily large.
In~\autoref{sec:kwise}, we propose a $k$-wise independence scheme that can provide the second type of guarantees by 
employing $O(\log^{d}\Delta)$ $k$-wise 
independent hash functions.
Its storage cost is quite small:  only $O(\log^{d}\Delta)$, which depends on neither $T$ nor $k$, for storing the seeds of these hash functions.
This $k$-wise independence scheme makes our $d$D-ERS solutions very practically useful for two reasons. 
First, such a $k$-wise independent hash function in practice requires a very short seed (not longer than a few kilobytes), and each hash operation can be computed in 
nanoseconds~\cite{univhash, tabulationpower}.
Finally, we emphasize that the issue of how strong this independence guarantee (among the underlying RVs) needs to be 
affects only the storage cost of our Gaussian-ERS and Poisson-ERS solutions, and is orthogonal all other issues described
in earlier paragraphs such as the $O(\log^d\Delta)$ time complexity of both solutions and 
the sufficient and likely necessary condition for a DST-based $d$D-ERS solution to exist. 


%  the time complexity of both solutions
%is always $O(\log^d\Delta)$ in both cases and hence is an orthogonal issue.


%$k$-wise independence scheme in~\autoref{sec:kwise}, which guarantees the underlying (Gaussian) RVs are $k$-wise independent using much less storage (which is independent of $T$). 
%For any $k > 1$,  the $k$-wise independence scheme needs to store only the seeds of $O(\log^{d}\Delta)$ instances of $k$-wise 
%independent hash functions.  



%$\vec{\mathbf{i}} \in  [0, \Delta)^d$\textbf{to generate the scalars in the aforementioned vector $\vec{\mathbf{w}}$ on demand}   ($X_{\vec{\mathbf{i}}}$)'s
\begin{comment}
In our solution, to provably guarantee that all the $\Delta^d$ underlying RVs  are independent, in theory we need to make an idealized assumption that we can map
every integer $i\in[0, \Delta^d)$ to a {\it fresh} RV $W_i$ (the $i^{th}$ scalar in the $\Delta^d$-dimensional $\vec{\mathbf{w}}$) independent of other RVs using a truly random hash function~\cite{mitzenmachertrulyrandom}.  
In practice, we can instantiate our solution to 
achieve three different levels of independence guarantees using three different types of more practically implementable hash functions, respectively.   
One such instantiation, called the $k$-wise independence scheme and to be elaborated in~\autoref{sec:kwise}, is another major contribution of this work.  
For any $k > 1$, the 
$k$-wise independence scheme can be configured, by employing $O(\log^{d}\Delta)$ $k$-wise 
independent hash functions to do this mapping (from $i$ to $W_i$), 
to guarantee that the underlying Gaussian RVs are $k$-wise independent.
\end{comment}
%requires a seed of only $O(\log\Delta)$ bits in length and has only $O(k)$ computational complexity per hashing operation.
%the  (per hashing operation) of  is only  
Second, most applications of ERS only require the underlying RVs to be 4-wise independent~\cite{onepasswavelet, muthukrishnanhistogram}. 
This $k$-wise independence scheme works also for our Poisson-ERS solution (described next).  We however will not explain how it works in this paper, since doing so would involve drilling down to 
the messy and lengthy detail of the Cartesian product of $d>1$ DSTs (since we cannot use the relatively clean and simple $d$D HWT in the Poisson case as just explained).
\textbf{Nisan??}

% although we have yet to find any practical application of the Poisson-ERS problem.

%We will describe two such applications in~\autoref{sec:introapplication}.

%Our Gaussian-ERS solution generalizes the DST-based approach to higher dimensions because, in 1D, a DST is mathematically equivalent to an HWT, as will be shown in~\autoref{sec:dst1D}.

% that we will describe in~\autoref{sec:2ddyasim}.

The contributions of this work can be summarized as follows.  First, we provide the first set of answers to the long-standing open question whether there is an efficient 
solution to {\it any} $d$D-ERS problem for $d > 1$.   Second, our Gaussian-ERS solution solves a long-standing open problem in data streaming
that we will describe next.
 %:to approximately answer, in an efficient manner, range-sum queries over a $d$-dimensional dynamic (subject to updates that arrive as a stream)  data cube for $d > 1$.  
Third, our $k$-wise independence theory and hashing scheme make our $d$D ERS solutions 
very practically useful.  

%one of which solves a long-standing open problem. 

The rest of the paper is organized as follows. In~\autoref{sec:introapplication}, we describe two applications of our $d$D Gaussian-ERS solutions.  In~\autoref{sec:dyasim}, we first describe our HWT-based Gaussian-ERS scheme in $1$D, and then generalize it to 2D and $d$D. In~\autoref{sec:kwise}, we describe our $k$-wise independence theory and scheme. In~\autoref{sec:infeasibility}, we propose a sufficient and likely necessary condition on the target distribution for the DST approach to be generalized to $d$D. Finally, we conclude the paper in~\autoref{sec:conclusion}.
%Although so far we only have efficient $d$D-ERS solutions for Gaussian and Poisson, 

%\textbf{Although our solution works only for these two nice distributions, we should feel blessed to have some results on this long-standing open problem of $d$D-ERS. }
%{\bf summarize the contributions here}

\begin{comment}
For all target distributions that satisfy this sufficient condition (including new ones we may discover
in the future), we propose a universal algorithmic framework 
that can be instantiated into a DST-based dD ERS solution for any such distribution.  

;  and for such target distributions (including new ones that 
we may discover
in the future)
this generalization  
We have also proposed a universal algorithmic framework that ``automates" this generaliz

dyadic simulation to be feasible in 2D (Condition (\ref{condindep})). Intuitively, this condition says the range-sums of horizontal and vertical strip-shaped ranges are conditionally independent given the sum of the entire universe. When the target distribution is Gaussian, this condition obviously holds, because horizontal and vertical wavelet coefficients are computed orthogonally. For other common distributions, we find that the condition above holds when the target distribution is Poisson, but does not hold when it is Cauchy or Rademacher. When Condition (\ref{condindep}) holds, we have a generalized dyadic simulation algorithm that solves 2D-ERS, but otherwise, dyadic simulation is likely infeasible on high dimensions, since it is not known how the naive dyadic simulation can be improved.


In 1D, our wavelet-based solution is equivalent to the Gaussian-DST, so a natural question is whether we can directly generalize dyadic simulation to solve multidimensional ERS on other target distributions that do not have a wavelet formulation.
%Starting from the wavelet-based solution above, we study the feasibility of generalizing the 1D-DST to solve multidimensional ERS for target distributions other than Gaussian.  In this study, we require the generated underlying RVs that are (at least empirically) independent.
Unfortunately, we find out that when we require the generated underlying RVs to be (at least empirically) independent, the ERS problem is significantly harder in even 2D than in 1D, and a naive generalization of dyadic simulation is clearly infeasible since it requires $O(\Delta)$ time and space.


Fortunately, we have characterized a sufficient condition for dyadic simulation to be feasible in 2D (Condition (\ref{condindep})). Intuitively, this condition says the range-sums of horizontal and vertical strip-shaped ranges are conditionally independent given the sum of the entire universe. When the target distribution is Gaussian, this condition obviously holds, because horizontal and vertical wavelet coefficients are computed orthogonally. For other common distributions, we find that the condition above holds when the target distribution is Poisson, but does not hold when it is Cauchy or Rademacher. When Condition (\ref{condindep}) holds, we have a generalized dyadic simulation algorithm that solves 2D-ERS, but otherwise, dyadic simulation is likely infeasible on high dimensions, since it is not known how the naive dyadic simulation can be improved.

\end{comment}

%In the scheme above, we have assumed the use of impractical truly random hash functions. By using $k$-wise independent hash functions instead,
%we provide a practical scheme in~\autoref{sec:kwise} that reduces the storage complexity to $O(\log^{d}\Delta)$ 
%while the underlying RVs are guaranteed to be $k$-wise independent. 

%Although both observations are already \textbf{separately} present in the literature~\cite{vershyninprobability, propolyne}, we are the first to realize they are closely related to the dyadic simulation scheme for Gaussian target distribution (Gaussian-DST for short) and lead to a $d$D-ERS solution. This point is critical, because it would be much easier
%to explain our Gaussian-ERS solution for higher dimensions using the wavelet language than using the DST language. 

%We are the first to find out that when the underlying RVs are Gaussian, the dyadic simulation solution (called Gaussian-DST) has the following equivalent formulation based on Haar wavelets: If the underlying RVs $X_0, X_1, \cdots, X_{\Delta-1}$ are viewed as a $\Delta$-dimensional vector $\mathbf{x}$, then $\mathbf{x}\triangleq H^{-1} \mathbf{w}$ is defined as the inverse discrete Haar wavelet transform (DHWT) (denoted by the inverse matrix $H^{-1}$) of a $\Delta$-dimensional vector $\mathbf{w}$ of i.i.d. standard Gaussian RVs. Given any range $[l, u)$, the range-sum $S[l, u)$ can be efficiently computed from $\mathbf{w}$ for the following reason. For ease of presentation, we define the \emph{indicator vector} $\mathbbm{1}_S$ of a set $S$ as follows: The $i^{th}$ element of $\mathbbm{1}_S$ is equal to $1$ if $i\in S$ and $0$ otherwise. Here, we let the set $S$ be the range $[l, u)$, and then the range-sum $S[l, u) = \sum_{i=l}^{u-1}X_i$ equals to the inner product $\langle \mathbf{x}, \mathbbm{1}_{[l, u)}\rangle$. Since DHWT is an orthogonal transform, it preserves the inner product between two vectors as shown in~\autoref{lem:orthoh}, so $S[l, u) = \langle H\mathbf{x}, H\mathbbm{1}_{[l, u)}\rangle = \langle \mathbf{w}, H\mathbbm{1}_{[l, u)}\rangle$. Therefore, the computation takes two steps.  First, the \emph{indicator vector}  $\mathbbm{1}_{[l, u)}$ is transformed to its wavelet coefficients $H\mathbbm{1}_{[l, u]}$ using the ``lazy wavelet transform''~\cite{propolyne}, which has logarithmic time complexity. Second, the range-sum $S[l, u)$ is computed as the inner product between $\mathbf{w}$ and $H\mathbbm{1}_{[l, u)}$. The second step is also efficient supposing any element of $\mathbf{w}$ can be accessed in constant time, because $H\mathbbm{1}_{[l, u)}$ only has a logarithmic number of nonzero elements.


%Although the 1D-DST solution is applicable to a wide range of target distributions, an equivalent wavelet formulation exists only for Gaussian distribution. This is because the wavelet transform from $\mathbf{w}$ to $\mathbf{x}$ is always linear, and Gaussian-DST is only dyadic simulation scheme that is known to be linear.

%, since  the transform  defined by the DST is linear for Gaussian distribution only, as required by the definition of wavelets.

% for other target distributions described in~\cite{1ddyadic}, the function that maps $\mathbf{w}$ to $\mathbf{x}$ would not even be a linear transform. (Wavelet transforms are always linear.) 


%As we will show in~\autoref{sec:dyasim}, the wavelet-based solution above naturally generalizes to two or more dimensions when the (fully separable) multidimensional DHWT~\cite{nievergeltwavelet} is used. With this solution, we can efficiently compute the range-sum of arbitrary $d$-dimensional rectangular ranges in $O(\log^d \Delta)$ time. % with a similar wavelet-based scheme in two or more dimensionspolylogarithmic time to $\Delta$. in~\autoref{sec:dyasim}.

%The multidimensional DHWT can be defined as the Kronecker product (a special form of tensor product) of several one-dimensional DHWTs $H^{(1)} \otimes H^{(2)} \otimes \cdots \otimes H^{(d)}$, in which $H^{(j)}$ denotes the DHWT on the $j^{th}$ dimension. Note that for any rectangular range in $[\Delta]^d$, in the form of $\{\mathbf{i}:\mathbf{l}\preceq \mathbf{i}\preceq \mathbf{u}\}$, its indicator vector $\mathbbm{1}_{\{\mathbf{i}:\mathbf{l}\preceq \mathbf{i}\preceq \mathbf{u}\}}$ can also be written as the Kronecker product of $d$ one-dimensional indicator vectors $\mathbbm{1}_{[l_1, u_1]}\otimes\mathbbm{1}_{[l_2, u_2]}\otimes\cdots\otimes \mathbbm{1}_{[l_d, u_d]}$.By the property of mixing Kronecker products and matrix products, in the first step of range-summability, the sparse representation of the range $\hat{\mathbf{r}}_{\mathbf{l},\mathbf{u}}$ equals to $(H^{(1)} \otimes H^{(2)} \otimes \cdots \otimes H^{(d)})\cdot (\mathbbm{1}_{[l_1, u_1]}\otimes\mathbbm{1}_{[l_2, u_2]}\otimes\cdots\otimes \mathbbm{1}_{[l_d, u_d]}) = (H^{(1)} \mathbbm{1}_{[l_1, u_1]})\otimes (H^{(2)} \mathbbm{1}_{[l_2, u_2]})\otimes\cdots\otimes(H^{(d)} \mathbbm{1}_{[l_d, u_d]})$, each of which is a one-dimensional sparse representation. This observation importantly shows that $\hat{\mathbf{r}}_{\mathbf{l},\mathbf{u}}$ can be factorized to the Kronecker product of $d$ one-dimensional sparse representations, so it issparse with a polylogarithmic number of nonzero elements. Therefore, both $\hat{\mathbf{r}}_{\mathbf{l},\mathbf{u}}$ and its inner product with $\mathbf{w}$ are computable in polylogarithmic time.  

%so the Kronecker product is sparse with polylogarithmic nonzeo elements and  to  without the aforementioned interference problem,  both efficiently computable in polylogarithmic time and  The latter property leads to the polylogarithmic time complexity of computing the inner product between $\hat{\mathbf{r}}_{\mathbf{l},\mathbf{u}}$ and $\mathbf{w}$ in the second step.

% which, as we will show in~\autoref{sec:infeasibility} is necessary for the ERS scheme to work in multiple dimensions.

%``independent enough'' for most of the applications.

%that we can access any element of a long random vector $\mathbf{w}$ of size $\Delta^d$ in constant time. However, this idealized case is impractical when the universe
%size $\Delta$ is massive, since 
%It is prohibitively expensive to generate a 
%massive number of fresh RVs since the (generated) 
%the value of each freshly generated RV would all have to be remembered (stored in memory) and there can be a massive number of them.   

%Our scheme first partitions the elements of $\mathbf{w}$, which can be regarded as $d$-dimensional DHWT coefficients, according to the scales $\mathbf{m}$ of the wavelet coefficients. For each scale $\mathbf{m}$, we use a $k$-wise independent (or off-the-shelf) hash function $h_{\mathbf{m}}(\cdot)$ to hash each index $\mathbf{j}$ in this partition to a standard Gaussian RV. When the random vector generated this way, denoted by $\mathbf{w}'$, is used instead of the standard Gaussian random vector $\mathbf{w}$, our scheme guarantees the $k$-wise (or empirical) independence of the underlying RVs, which extends the strong independence guarantees of dyadic simulation to multi-dimensional universes.

% can be first separately computed on each dimension, and then taking the Kronecker product of $d$ sparse vectors that each has $O(\log \Delta)$ nonzero elements.


%Since the DHWT has already been generalized to multiple dimensions in the data streaming literature, relies on the following property of : 



%==============================

%\subsection{Feasibility of $d$D-ERS for General Target Distributions}\label{sec:intro-infeasible}


%Although $1$D-ERS on general target distributions is readily solved by dyadic simulation~\cite{1ddyadic}, $2$D-ERS is likely to remain infeasible for dyadic simulation unless the target distribution has a ``nice'' special conditional independence property specified below. %guaranteeing the ( independence of underlying RVs 


 %We focus on the dyadic simulation approach, because this is the only approach that guarantees empirical independence of general underlying distributions on one dimension~\cite{1ddyadic}. 


 %$S^V_j$ is conditionally independent to each $S^H$ given their sum  $S^H_0+S^H_1+\dots+S^H_{\Delta-1}$. If this condition holds, only a single sum needs to be memorized that encodes all the dependency between $S^V_j$ and the horizontal strips, which is exactly the range-sum of the universe generated at the beginning of dyadic simulation. However, this nice conditional independence does not hold for all target distributions. As we will show in~\autoref{sec:infeasibility}, it holds for Gaussian or Poisson distribution, but not for Cauchy or Bernoulli.  Since it is not known how find a similar alternative to encode the vast information in these $\Delta$ horizontal stripes, Condition~(\ref{condindep}) is likely to be also a necessary condition for dyadic simulation to be feasible on a  multidimensional universe, even if approximately.


% As we will show in~\autoref{prop:condnindep}, under ,  without any form of conditional independence, so conditional independence rule 


% : Any , which , can be split into $O(\log^2 \Delta)$ dyadic rectangles, defined as the Cartesian product of two dyadic ranges.ERS is an important problem in data streaming, w


%\subsection{Applications}






